AI Competitions and Benchmarks: Dataset Development

Machine learning is now used in many applications thanks to its ability to predict, generate, or discover patterns from large quantities of data. However, the process of collecting and transforming data for practical use is intricate. Even in today's digital era, where substantial data is generated daily, it is uncommon for it to be readily usable; most often, it necessitates meticulous manual data preparation. The haste in developing new models can frequently result in various shortcomings, potentially posing risks when deployed in real-world scenarios (eg social discrimination, critical failures), leading to the failure or substantial escalation of costs in AI-based projects. This chapter provides a comprehensive overview of established methodological tools, enriched by our practical experience, in the development of datasets for machine learning. Initially, we develop the tasks involved in dataset development and offer insights into their effective management (including requirements, design, implementation, evaluation, distribution, and maintenance). Then, we provide more details about the implementation process which includes data collection, transformation, and quality evaluation. Finally, we address practical considerations regarding dataset distribution and maintenance.

==> glossary.tex <==
%%% words/definitions
% in text use: \gls{task}

\newglossaryentry{coopetition}{
    name={coopetition},
    description={TODO}
}

\newglossaryentry{classification}{
    name={classification},
    description={A \gls{supervised-learning} task  in which labels are categorical variables (discrete, usually non ordinal).}
}

\newglossaryentry{regression}{
    name={regression},
    description={A \gls{supervised-learning} task in which labels are continuous or ordinal (categorical regression).}
}

\newglossaryentry{dataset}{%
  name={dataset},%
  description={A collection of labeled or unlabeled \gls{data-samples}.}%
  }

\newglossaryentry{dataset-requirements}{
    name={dataset requirements},
    description={The set of specifications of a dataset outlined in a document drafted before and collection begins. It should include, among other things, nature of the data, purpose, quality and quantity, means, costs, timeline.}
}

\newglossaryentry{dataset-design}{%
  name={dataset design},%
  description={The formal definition of a particular \gls{data-collection}.}.
  }
  
\newglossaryentry{dataset-implementation}{%
  name={dataset implementation},%
  description={Carrying out a particular \gls{data-collection} according to a given \gls{dataset-design}.}.
  }
  
\newglossaryentry{dataset-life-cycle}{
    name={dataset life-cycle},
    description={The set of processes which creates or transforms a dataset from \gls{dataset-requirements} to its \gls{dataset-distribution} and \gls{dataset-maintenance} or \gls{dataset-deprecation}.}
}

%%% data KEYWORD

\newglossaryentry{data-collection}{
    name={data collection},
    description={The set of processes involved in producing a \gls{dataset}.}
}

\newglossaryentry{data-gathering}{
    name={data gathering},
    description={A particular \gls{data-collection}, which consists in gathering existing \gls{data-samples} or an entire existing \gls{dataset}, possibly from different sources, on which we do not have any influence.}
}

\newglossaryentry{data-reusing}{
    name={data reusing},
    description={The action of using an existing \gls{dataset} in an application, without changing its original purpose. Reusing is distinct from \gls{data-repurposing} or \gls{data-recycling}.}
}

\newglossaryentry{data-repurposing}{
    name={data repurposing},
    description={The action of using an existing \gls{dataset} in a new task or application, by changing its original purpose. Repurposing may include changing \gls{data-annotation}, re-sampling, transforming. Repurposing is distinct from \gls{data-reusing} or \gls{data-recycling}.}
}

\newglossaryentry{data-recycling}{
    name={data recycling },
    description={A particular \gls{data-collection}, which consists in recycling existing \gls{data-samples} or an entire existing \gls{dataset}, possibly from different sources, on which we do not have any influence. Recycling is distinct from \gls{data-reusing} or \gls{data-repurposing}.}
}

\newglossaryentry{data-resampling}{
    name={data resampling},
    description={The action selecting particular \gls{data-samples} in a \gls{dataset}. This may yield \gls{sample-bias} (or correct it).}
}

\newglossaryentry{data-synthesis}{
    name={data synthesis or generation},
    description={Is the process of generating artificial data that mimics real-world observations and can be used to (pre)train machine learning models when actual data is difficult or expensive to get.}
}

\newglossaryentry{data-bias}{
    name={data bias},
    description={The existence of spurious correlations (or dependencies) between data labels \gls{spurious-feature}s. Data bias includes \gls{sample-bias} and \gls{confounding-bias}}
}

\newglossaryentry{sample-bias}{
    name={sample bias},
    description={A particular type of \gls{data-bias} induced by selecting samples in a non-representative way of the target population.}
}

\newglossaryentry{confounding-bias}{
    name={confounding bias},
    description={A particular type of \gls{data-bias} induced by the existence of a common cause between labels and \gls{spurious-feature}s.}
}

\newglossaryentry{spurious-feature}{
    name={spurious feature},
    description={A variable (or feature or attribute) of \gls{data-samples}, which may be a ``protected attribute'' that could trigger discrimination (\eg gender, ethnicity, or age) or a variable known to be irrelevant to the particular task at hand (\eg the identity of the data collector, the time of data collection, the recording conditions).}
}

\newglossaryentry{core-feature}{
    name={core feature},
    description={A variable (or feature or attribute), which is though of as ``leggitimate'' to use to perform a \gls{learning-task}, as opposed to a \gls{spurious-feature}. Note that it is possible, because of \gls{entanglement} that some variable in a \gls{data-represention} combine original spurious and core features. Merely suppressing spurious features may not resolve the problem of bias in data.}
}


\newglossaryentry{data-simulation}{
    name={data simulation},
    description={A particular \gls{data-collection}, which consists in artificially creating data with a numerical simulator.}
}

\newglossaryentry{data-acquisition}{
    name={data acquisition},
    description={A particular \gls{data-collection}, which consists in measuring a real world signal with instruments, and converting it to digital information.}
}

\newglossaryentry{data-annotation}{
    name={data annotation},
    description={The action of attaching to existing data another type of complementary data, often called \gls{meta-data}, providing extra information (\eg object bounding boxes).}
}

\newglossaryentry{meta-data}{
    name={meta-data},
    description={Various \gls{data-annotation}s providing extra information to \gls{data-samples} (\eg object bounding boxes, date and time of collection, data origin).}
}


\newglossaryentry{data-labelling}{
    name={data labelling},
    description={A particular \gls{data-annotation}, which consists in mapping data samples to class labels. By extension, in the case of regression, labels can be continuous variables.}
}

\newglossaryentry{data-samples}{
    name={data samples},
    description={Individual units in a dataset.}
}

\newglossaryentry{data-transformation}{
    name={data transformation},
    description={A set of processes, which map an input data representation to an output data representation.}
}

\newglossaryentry{data-augmentation}{
    name={data augmentation},
    description={A set of processes which generates new data samples based on a fixed input dataset.}
}

\newglossaryentry{data-integration}{
    name={data integration},
    description={A set of processes which merge different datasets with complementary properties such as features, sources or quantities.}
}

\newglossaryentry{data-fusion}{
    name={data fusion},
    description={Synonym of data-integration.}
}

\newglossaryentry{data-cleaning}{
    name={data cleaning},
    description={A set of processes which detect, remove or replace mistakes in data samples.}
}

\newglossaryentry{data-reduction}{
    name={data reduction},
    description={Set of processes that reduce the quantity of information contained in a dataset for example to have improve computational efficiency or to reduce noise.}
}

\newglossaryentry{data-representation}{
    name={data representation},
    description={A well specified data structure in which each \gls{data-samples} is stored in a digital form in a computer. Feature vectors are a frequently used data representation in Machine Learning.}
}

\newglossaryentry{data-normalization}{
    name={data normalization},
    description={Set of processes that harmonizes or homogenizes representations of data.}
}

\newglossaryentry{data-calibration}{
    name={data calibration},
    description={Set of processes that ensure the correctness of collected data in average.}
}

\newglossaryentry{dataset-evaluation}{
    name={dataset evaluation},
    description={A set of processes, which verify that the produced \gls{dataset} meets the \gls{dataset-requirements}.}
}

\newglossaryentry{dataset-distribution}{
    name={dataset distribution},
    description={Means of making a \gls{dataset} available to the public.}
}

\newglossaryentry{dataset-maintenance}{
    name={dataset maintenance},
    description={Means of ensuring error corrections, upgrades, user-feedback, new regulations, or new ethical standards, are incorporated into new versions of the dataset.}
}

\newglossaryentry{dataset-retirement}{
    name={dataset retirement},
    description={Retiring a \gls{dataset} from public availability because of irreversible errors, new regulations, or new ethical standards.}
}

\newglossaryentry{dataset-deprecation}{
    name={dataset deprecation},
    description={Notification that a \gls{dataset} should not be used anymore but remains public for traceability or restricted usage because of irreversible errors, new regulations, or new ethical standards.}
}

\newglossaryentry{data-soundness}{
    name={data soundness},
    description={...}
}

\newglossaryentry{data-completeness}{
    name={data completeness},
    description={...}
}

\newglossaryentry{data-compactness}{
    name={data compactness},
    description={...}
}

\newglossaryentry{learning-task}{%
  name={learning task},%
  description={A formal prediction problem, denoted as $T$, composed of \gls{training-data} and \gls{validation-data} or \gls{test-data}, depending on the challenge phase, with the objective of (1) producing a \gls{predictor} using a \gls{trainer} (supplied by a challenge participant) using training data, and (2) evaluating the \gls{predictor}, using validation or test data. The evaluation is carried out using one (or several) \gls{evaluation-metric}s.}%
}

\newglossaryentry{evaluation-metric}{%
  name={evaluation metric},%
  description={A function $L(\hat{y}, y)$, of a prediction  $\hat{y}=f(x)$ made by a \gls{predictor} $f(.)$ on a input sample $x$ (from \gls{validation-data} or \gls{test-data}) and an associated ``ground truth'' value $y$. A score is obtained by averaging $L(\hat{y}, y)$ over all validation of test samples, which estimates empirically the generalization performance of the predictor. }
  }

\newglossaryentry{training-data}{%
  name={training data},%
  description={A subset of the \gls{dataset} $D_{tr} = \{ (x_i, y_i) \}_{i=1}^n \subseteq X \times Y$, which represent a snapshot of the ``real-world'', assumed to be drawn from a probability distribution $P$ on $X \times Y$, which represents the abstract process generating the data (usually unknown). This subset is used by the \gls{trainer} (or learning algorithm).}%
}

\newglossaryentry{validation-data}{%
  name={validation data},%
  description={A subset of the \gls{dataset}, disjoint from the \gls{training-data}, but usually drawn from the same distribution, used to get feed-back on performance during the development of a learning algorithm, so the \gls{test-data} remains untouched until the final evaluation. Using test data to adjust hyper-parameters of select algorithms results in optimistically biased performances. In a challenge, validation data are used for evaluation during the \gls{development-phase} (or feed-back phase).}%
}

\newglossaryentry{warmup-phase}{%
  name={warmup phase},%
  description={A challenge phase (also called public phase or challenge beta-testing) during which the participants are invited to try out the challenge protocol before the official starting date of the \gls{development-phase}, using some sample (public) data, not used in subsequent phases.}
  }

\newglossaryentry{development-phase}{%
  name={development phase},%
  description={A challenge phase (also called feed-back phase), during which the participants develop a solution to the problem of the challenge and submit results for immediate evaluation on \gls{validation-data}, to received feed-back on a (public) leaderboard.}
  }
  
  \newglossaryentry{final-phase}{%
  name={final phase},%
  description={A challenge phase (also called final test phase), during which the participants are evaluated on \gls{test-data}, not used either for training or validation. The final phase leaderboard remains private (only visible to the organizers) until the challenge is over.}
  }
  
\newglossaryentry{test-data}{%
  name={test data},%
  description={A subset of the \gls{dataset}, disjoint from the \gls{training-data} and the \gls{validation-data}, used to get feed-back on performance during the development of a learning algorithm, so the \gls{test-data} remains untouched until the final evaluation. Using test data to adjust hyper-parameters of select algorithms results in optimistically biased performances. In a challenge, test data are used for evaluation only once (for each final entry of each participant) in the \gls{final-phase}.}%
}

\newglossaryentry{alpha-challenge}{%
  name={$\alpha$-challenge},%
  description={}%
}

\newglossaryentry{beta-challenge}{%
  name={$\beta$-challenge},%
  description={}%
}

\newglossaryentry{predictor}{%
  name={predictor},%
  description={A function $f(.)$ mapping an input $x$ to an output $y$, solving a {classification} or a \gls{regression} problem. An \gls{alpha-challenge} asks participants to submit (trained) predictors.}%
}

\newglossaryentry{trainer}{%
  name={trainer},%
  description={An algorithm (usually called learning algorithm), which outputs a \gls{predictor}, or more generally a trained learning machine, which may be a data generator. The input to a trainer is \gls{training-data}. A \gls{beta-challenge} asks participants to submit trainers, and eventually tests on multiple \gls{learning-task}s their capability of automated machine learning (AutoML).}%
}

\newglossaryentry{meta-trainer}{%
  name={meta trainer},%
  description={An algorithm, which outputs a \gls{trainer}, given a dataset of datasets (meta-training set). A \gls{gamma-challenge} asks participants to submit meta-trainers, and tests on a meta-test set their capability of learning to learn (meta-learning).}%
}

\newglossaryentry{supervised-learning}{
    name={supervised learning},
    description={A \gls{learning-task} in which labels $Y$ are specified.}
}

\newglossaryentry{power-differential}{
    name={power differential},
    description={The difference in power between persons in positions of authority and those individuals in subordinate positions, which results in a vulnerability on the part of the subordinate. For example, the natural differences in power that exist between faculty and student.}
}

\newglossaryentry{observational-setting}{
    name={observational setting},
    description={A method for collecting data in which the investigator in charge of data collection does not interfere with the phenomenon. The distribution of samples collected should reflect the ``natural'' distribution of data.}
}

\newglossaryentry{experimental-setting}{
    name={experimental setting},
    description={A method for collecting data in which  the investigator  interferes with the natural world to achieve desired effects. A planned experiment consists in varying some factors systematically, in a controlled manner, or randomly.}
}

  
%%% acronyms
% in text use: \glspl{tla}

\newacronym{dlc}{DLC}{Data Life-Cycle}

\newacronym{ddlc}{DDLC}{Dataset Development Life-Cycle}

\newacronym{gdpr}{GDPR}{General Data-Protection Regulation}

\newacronym{mllc}{MLLC}{Machine Learning Life-Cycle}

\newacronym{sari}{SARI}{State Action Reward Information}

\newacronym{dream}{DREAM}{Dialogue for Reverse Engineering Assessment and Methods}

\newacronym{casp}{CASP}{Critical Assessment of protein Structure Prediction}

\newacronym{miccai}{MICCAI}{Medical Image Computing and Computer Assisted Intervention Society}

==> ref.bib.bkp.2 <==
@ARTICLE{8862913,
  author={Roh, Yuji and Heo, Geon and Whang, Steven Euijong},
  journal={IEEE Transactions on Knowledge and Data Engineering}, 
  title={A Survey on Data Collection for Machine Learning: A Big Data - {AI} Integration Perspective}, 
  year={2021},
  volume={33},
  number={4},
  pages={1328-1347},
  doi={10.1109/TKDE.2019.2946162}
}



@article{richard2024ai,
  author       = {Magali Richard and
                  Yuna Blum and
                  Justin Guinney and
                  Gustavo Stolovitzky and
                  Adrien Pav{\~{a}}o},
  title        = {{AI} Competitions and Benchmarks, Practical issues: Proposals, grant
                  money, sponsors, prizes, dissemination, publicity},
  journal      = {CoRR},
  volume       = {abs/2401.04452},
  year         = {2024},
}



@InProceedings{baz2021metadl,
  title = 	 {MetaDL challenge design and baseline results},
  author =       {El Baz, Adrian and Guyon, Isabelle and Liu, Zhengying and van Rijn, Jan N. and Treguer, Sebastien and Vanschoren, Joaquin},
  booktitle = 	 {AAAI Workshop on Meta-Learning and MetaDL Challenge},
  pages = 	 {1--16},
  year = 	 {2021},
  editor = 	 {Guyon, Isabelle and van Rijn, Jan N. and Treguer, Sébastien and Vanschoren, Joaquin},
  volume = 	 {140},
  series = 	 {Proceedings of Machine Learning Research},
  publisher =    {PMLR}
}

@book{brazdil2022metalearning,
  title={Metalearning: Applications to Automated Machine Learning and Data Mining},
  author={Brazdil, P and van Rijn, Jan N. and Soares, Carlos and Vanschoren, Joaquin},
  year = {2022},
  edition = {2nd},
  publisher = {Springer}
}


@article{huisman2021survey,
  title={A survey of deep meta-learning},
  author={Huisman, Mike and van Rijn, Jan Nicolaas and Plaat, Aske},
  journal={{Artificial Intelligence Review}},
  pages={1--59},
  year={2021},
  publisher={Springer}
}

@article{DBLP:journals/corr/abs-2010-04053,
  author    = {Simon Caton and
               Christian Haas},
  title     = {Fairness in Machine Learning: {A} Survey},
  journal   = {CoRR},
  volume    = {abs/2010.04053},
  year      = {2020},
  url       = {https://arxiv.org/abs/2010.04053},
  archivePrefix = {arXiv},
  eprint    = {2010.04053},
  timestamp = {Tue, 13 Oct 2020 15:25:23 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-2010-04053.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{mohr2021fast,
  author    = {Felix Mohr and
               Jan N. van Rijn},
  title     = {Fast and Informative Model Selection using Learning Curve Cross-Validation},
  journal   = {CoRR},
  volume    = {abs/2111.13914},
  year      = {2021},
}

@book{chin2004agile,
  title={Agile Project Management: How to Succeed in the Face of Changing Project Requirements},
  author={Chin, G.},
  isbn={9780814427361},
  year={2004},
  publisher={AMACOM}
}

@article{DBLP:journals/corr/abs-1908-09635,
  author    = {Ninareh Mehrabi and
               Fred Morstatter and
               Nripsuta Saxena and
               Kristina Lerman and
               Aram Galstyan},
  title     = {A Survey on Bias and Fairness in Machine Learning},
  journal   = {CoRR},
  volume    = {abs/1908.09635},
  year      = {2019},
  url       = {http://arxiv.org/abs/1908.09635},
  archivePrefix = {arXiv},
  eprint    = {1908.09635},
  timestamp = {Thu, 29 Aug 2019 16:32:34 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-1908-09635.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@InProceedings{Birhane_2021_WACV,
    author    = {Birhane, Abeba and Prabhu, Vinay Uday},
    title     = {Large Image Datasets: A Pyrrhic Win for Computer Vision?},
    booktitle = {Proceedings of the IEEE/CVF Winter Conference on Applications of Computer Vision (WACV)},
    month     = {January},
    year      = {2021},
    pages     = {1537-1547}
}

@inproceedings{10.1145/3351095.3372829,
author = {Jo, Eun Seo and Gebru, Timnit},
title = {Lessons from Archives: Strategies for Collecting Sociocultural Data in Machine Learning},
year = {2020},
isbn = {9781450369367},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/3351095.3372829},
doi = {10.1145/3351095.3372829},
booktitle = {Proceedings of the 2020 Conference on Fairness, Accountability, and Transparency},
pages = {306–316},
numpages = {11},
keywords = {archives, datasets, sociocultural data, ML fairness, data collection, machine learning},
location = {Barcelona, Spain},
series = {FAT* '20}
}


@article{10.1145/3458723,
author = {Gebru, Timnit and Morgenstern, Jamie and Vecchione, Briana and Vaughan, Jennifer Wortman and Wallach, Hanna and III, Hal Daum\'{e} and Crawford, Kate},
title = {Datasheets for datasets},
year = {2021},
issue_date = {December 2021},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
volume = {64},
number = {12},
issn = {0001-0782},
abstract = {Documentation to facilitate communication between dataset creators and consumers.},
journal = {Commun. ACM},
month = {nov},
pages = {86–92},
numpages = {7}
}



@article{DBLP:journals/corr/abs-1908-06165,
  author    = {Timnit Gebru},
  title     = {Oxford Handbook on {AI} Ethics Book Chapter on Race and Gender},
  journal   = {CoRR},
  volume    = {abs/1908.06165},
  year      = {2019},
  url       = {http://arxiv.org/abs/1908.06165},
  archivePrefix = {arXiv},
  eprint    = {1908.06165},
  timestamp = {Mon, 26 Aug 2019 13:20:40 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-1908-06165.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{10.1145/3375627.3375820,
author = {Raji, Inioluwa Deborah and Gebru, Timnit and Mitchell, Margaret and Buolamwini, Joy and Lee, Joonseok and Denton, Emily},
title = {Saving Face: Investigating the Ethical Concerns of Facial Recognition Auditing},
year = {2020},
isbn = {9781450371100},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/3375627.3375820},
doi = {10.1145/3375627.3375820},
location = {New York, NY, USA},
series = {AIES '20}
}

@inproceedings{10.1145/3287560.3287596,
author = {Mitchell, Margaret and Wu, Simone and Zaldivar, Andrew and Barnes, Parker and Vasserman, Lucy and Hutchinson, Ben and Spitzer, Elena and Raji, Inioluwa Deborah and Gebru, Timnit},
title = {Model Cards for Model Reporting},
year = {2019},
isbn = {9781450361255},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/3287560.3287596},
doi = {10.1145/3287560.3287596},
booktitle = {Proceedings of the Conference on Fairness, Accountability, and Transparency},
pages = {220–229},
numpages = {10},
location = {Atlanta, GA, USA},
series = {FAT* '19}
}

@inproceedings{wan2016chalearn,
  title={Chalearn looking at people rgb-d isolated and continuous datasets for gesture recognition},
  author={Wan, Jun and Zhao, Yibing and Zhou, Shuai and Guyon, Isabelle and Escalera, Sergio and Li, Stan Z},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition Workshops},
  pages={56--64},
  year={2016}
}

@inproceedings{molchanov2016online,
  title={Online detection and classification of dynamic hand gestures with recurrent 3d convolutional neural network},
  author={Molchanov, Pavlo and Yang, Xiaodong and Gupta, Shalini and Kim, Kihwan and Tyree, Stephen and Kautz, Jan},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={4207--4215},
  year={2016}
}

@article{sincan2020autsl,
  title={Autsl: A large scale multi-modal turkish sign language dataset and baseline methods},
  author={Sincan, Ozge Mercanoglu and Keles, Hacer Yalim},
  journal={IEEE Access},
  volume={8},
  pages={181340--181355},
  year={2020},
  publisher={IEEE}
}

@inproceedings{lin2014microsoft,
  title={Microsoft coco: Common objects in context},
  author={Lin, Tsung-Yi and Maire, Michael and Belongie, Serge and Hays, James and Perona, Pietro and Ramanan, Deva and Doll{\'a}r, Piotr and Zitnick, C Lawrence},
  booktitle={European conference on computer vision},
  pages={740--755},
  year={2014},
  organization={Springer}
}

@article{voigt2017eu,
  title={The eu general data protection regulation (gdpr)},
  author={Voigt, Paul and Von dem Bussche, Axel},
  journal={A Practical Guide, 1st Ed., Cham: Springer International Publishing},
  volume={10},
  pages={3152676},
  year={2017},
  publisher={Springer}
}

@article{daoli33situation,
  title={Situation, Dilemma and Countermeasures of China's Data Security Legislation: Comment on the Data Security Law of the People's Republic of China (Draft)},
  author={Daoli, HUANG and Wenhua, HU},
  journal={Journal of Beijing University of Aeronautics and Astronautics Social Sciences Edition},
  volume={33},
  number={6},
  pages={9}
}




@ARTICLE{Roh:2021,
  author={Roh, Yuji and Heo, Geon and Whang, Steven Euijong},
  journal={IEEE Transactions on Knowledge and Data Engineering}, 
  title={A Survey on Data Collection for Machine Learning: A Big Data - AI Integration Perspective}, 
  year={2021},
  volume={33},
  number={4},
  pages={1328-1347}
}

@article{Zhang:2016,
	author = {Zhang, Jing and Wu, Xindong and Sheng, Victor S.},
	title = {Learning from Crowdsourced Labeled Data: A Survey},
	year = {2016},
	publisher = {Kluwer Academic Publishers},
	address = {USA},
	volume = {46},
	number = {4},
	journal = {Artificial Intelligence Review},
	pages = {543-576}
}

@article{Shorten:2019,
	author = {Shorten, Connor and Khoshgoftaar, Taghi},
	year = {2019},
	month = {07},
	pages = {},
	title = {A survey on Image Data Augmentation for Deep Learning},
	volume = {6},
	journal = {Journal of Big Data},
	doi = {10.1186/s40537-019-0197-0}
}

@article{Engelen:2020,
	author = {Engelen, Jesper and Hoos, Holger},
	year = {2020},
	month = {02},
	pages = {373-440},
	title = {A survey on semi-supervised learning},
	volume = {109},
	journal = {Machine Learning},
	doi = {10.1007/s10994-019-05855-6}
}

@INPROCEEDINGS{Deng:2009,
	author={Deng, Jia and Dong, Wei and Socher, Richard and Li, Li-Jia and Kai Li and Li Fei-Fei},
	booktitle={2009 IEEE Conference on Computer Vision and Pattern Recognition}, 
	title={ImageNet: A large-scale hierarchical image database}, 
	year={2009},
	pages={248-255}
}

@ARTICLE{Zhang:PAMI:2021,
	author={Zhang, Dingwen and Han, Junwei and Cheng, Gong and Yang, Ming-Hsuan},
	journal={IEEE Transactions on Pattern Analysis and Machine Intelligence (TPAMI)}, 
	title={Weakly Supervised Object Localization and Detection: A Survey}, 
	year={2021}
}

@ARTICLE{Escalante:TAC:2020,
	author={Escalante, Hugo Jair and Kaya, Heysem and Salah, Albert Ali and Escalera, Sergio and G{\"{u}}{\c{c}}l{\"{u}}t{\"{u}}rk, Yağmur and G{\"{u}}{\c{c}}l{\"{u}}, Umut and Bar\'o, Xavier and Guyon, Isabelle and Jacques, Julio C. S. and Madadi, Meysam and Ayache, Stephane and Viegas, Evelyne and Gurpinar, Furkan and Wicaksana, Achmadnoer Sukma and Liem, Cynthia and Van Gerven, Marcel A. J. and Van Lier, Rob},
	journal={IEEE Transactions on Affective Computing}, 
	title={Modeling, Recognizing, and Explaining Apparent Personality from Videos}, 
  year={2020},
  volume={13},
  number={2},
  pages={894-911},
}

@InProceedings{Junior_2021_WACV,
	author    = {{Jacques Junior}, Julio C. S. and Lapedriza, Agata and Palmero, Cristina and Baro, Xavier and Escalera, Sergio},
	title     = {Person Perception Biases Exposed: Revisiting the First Impressions Dataset},
	booktitle = {IEEE/CVF Winter Conference on Applications of Computer Vision Workshops},
	year      = {2021},
	pages     = {13-21}
}

@article{Zhao:2017,
	author    = {Jieyu Zhao and
	Tianlu Wang and
	Mark Yatskar and
	Vicente Ordonez and
	Kai{-}Wei Chang},
	title     = {Men Also Like Shopping: Reducing Gender Bias Amplification using Corpus-level
	Constraints},
	journal   = {CoRR},
	volume    = {abs/1707.09457},
	year      = {2017},
	archivePrefix = {arXiv},
	eprint    = {1707.09457}
}

@InProceedings{Hendricks_2018_ECCV,
	author = {Anne Hendricks, Lisa and Burns, Kaylee and Saenko, Kate and Darrell, Trevor and Rohrbach, Anna},
	title = {Women also Snowboard: Overcoming Bias in Captioning Models},
	booktitle = {The European Conference on Computer Vision (ECCV)},
	month = {September},
	year = {2018}
} 

@ARTICLE{dario:TAC:2019,
	author={R. D. {P\'erez Principi} and C. {Palmero} and Julio C. S. {Jacques Junior} and S. {Escalera}},
	journal={IEEE Transactions on Affective Computing},
	title={On the Effect of Observed Subject Biases in Apparent Personality Analysis from Audio-visual Signals},
	year={2019},
	pages={1-14}
}

@InProceedings{Wang_2019_ICCV,
	author = {Wang, Tianlu and Zhao, Jieyu and Yatskar, Mark and Chang, Kai-Wei and Ordonez, Vicente},
	title = {Balanced Datasets Are Not Enough: Estimating and Mitigating Gender Bias in Deep Image Representations},
	booktitle = {Proceedings of the IEEE/CVF International Conference on Computer Vision (ICCV)},
	month = {October},
	year = {2019}
}

@article{Wang:NLP:2020,
	author = {Wang, Shirui and Zhou, Wenan and Jiang, Chao},
	year = {2020},
	month = {03},
	pages = {},
	title = {A survey of word embeddings based on deep learning},
	volume = {102},
	journal = {Computing},
	doi = {10.1007/s00607-019-00768-7}
}

@inproceedings{Liu:IJCAI:2018,
	author = {Liu, Yun and Jiang, Peng-Tao and Petrosyan, Vahan and Li, Shi-Jie and Bian, Jiawang and Zhang, Le and Cheng, Ming-Ming},
	title = {DEL: Deep Embedding Learning for Efficient Image Segmentation},
	year = {2018},
	isbn = {9780999241127},
	publisher = {AAAI Press},
	booktitle = {Proceedings of the 27th International Joint Conference on Artificial Intelligence},
	pages = {864-870},
	location = {Stockholm, Sweden},
	series = {IJCAI'18}
}

@InProceedings{Tang:DSAA:2021,
author="Tang, Xiu
and Wu, Sai
and Chen, Gang
and Chen, Ke
and Shou, Lidan",
editor="Jensen, Christian S.
and Lim, Ee-Peng
and Yang, De-Nian
and Lee, Wang-Chien
and Tseng, Vincent S.
and Kalogeraki, Vana
and Huang, Jen-Wei
and Shen, Chih-Ya",
title="Learning to Label with Active Learning and Reinforcement Learning",
booktitle="Database Systems for Advanced Applications",
year="2021",
publisher="Springer International Publishing",
pages="549--557",
isbn="978-3-030-73197-7"
}

@inproceedings{bischl2021openml,
  Author 	= {B. Bischl and G. Casalicchio and M. Feurer and P. Gijsbers and F. Hutter and M. Lang and R. G. Mantovani and J. N. van Rijn and J. Vanschoren},
  Title 	= {{OpenML} Benchmarking Suites},
  Year 		= {2021},
  booktitle = {Proceedings of the Neural Information Processing Systems Track on Datasets and Benchmarks}}

@article{fisher1936use,
  title={The use of multiple measurements in taxonomic problems},
  author={Fisher, Ronald A},
  journal={Annals of eugenics},
  volume={7},
  number={2},
  pages={179--188},
  year={1936},
  publisher={Wiley Online Library}
}

@article{gijsbers2019open,
  title={An open source AutoML benchmark},
  author={Gijsbers, Pieter and LeDell, Erin and Thomas, Janek and Poirier, S{\'e}bastien and Bischl, Bernd and Vanschoren, Joaquin},
  journal={arXiv preprint arXiv:1907.00909},
  year={2019}
}

@techreport{geva1992cart,
author = {Geva, Shlomo and Sitte, Joaquin},
title = {The Cart-Pole Experiment as a Benchmark for Trainable Controllers},
year = {1992},
publisher = {University of Queensland},
address = {AUS},
}

@INPROCEEDINGS{guyon2015design,
 author={I. Guyon and K. Bennett and G. Cawley and H. J. Escalante and S. Escalera and Tin Kam Ho and N. Macià and B. Ray and M. Saeed and A. Statnikov and E. Viegas},
 booktitle={2015 International Joint Conference on Neural Networks (IJCNN)},
 title={Design of the 2015 ChaLearn AutoML challenge},
 year={2015},
 pages={1-8},
 ISSN={2161-4393}
}

@article{krizhevsky2012imagenet,
  title={Imagenet classification with deep convolutional neural networks},
  author={Krizhevsky, Alex and Sutskever, Ilya and Hinton, Geoffrey E},
  journal={Advances in neural information processing systems},
  volume={25},
  pages={1097--1105},
  year={2012}
}

@article{lake2019omniglot,
  title={The Omniglot challenge: a 3-year progress report},
  author={Lake, Brenden M and Salakhutdinov, Ruslan and Tenenbaum, Joshua B},
  journal={Current Opinion in Behavioral Sciences},
  volume={29},
  pages={97--104},
  year={2019},
  publisher={Elsevier}
}

@inproceedings{lindauer2017open,
  title={Open algorithm selection challenge 2017: Setup and scenarios},
  author={Lindauer, Marius and van Rijn, Jan N and Kotthoff, Lars},
  booktitle={Open Algorithm Selection Challenge 2017},
  pages={1--7},
  year={2017},
  organization={PMLR}
}

@article{lindauer2019algorithm,
  title={The algorithm selection competitions 2015 and 2017},
  author={Lindauer, Marius and van Rijn, Jan N and Kotthoff, Lars},
  journal={Artificial Intelligence},
  volume={272},
  pages={86--100},
  year={2019},
  publisher={Elsevier}
}


@article{mcdermott2016diagnosing,
  title={Diagnosing a disorder in a classification benchmark},
  author={McDermott, James and Forsyth, Richard S},
  journal={Pattern Recognition Letters},
  volume={73},
  pages={41--43},
  year={2016},
  publisher={Elsevier}
}

@inproceedings{palacios2021automated,
    author = {Palacios Salinas, Nelly Rosaura and Baratchi, Mitra and van Rijn, Jan N. and Vollrath, Andreas},
    title = "Automated Machine Learning for Satellite Data: Integrating Remote Sensing Pre-trained Models into AutoML Systems",
    booktitle = "Proceedings of the European Conference on Machine Learning and Principles and Practice of Knowledge Discovery in Databases",
    series = {ECML/PKDD 2021},
    year = "2021"
}


@article{mohr2022learning,
  author    = {Felix Mohr and Jan N. van Rijn},
  title     = {Learning Curves for Decision Making in Supervised Machine Learning - {A} Survey},
  journal   = {CoRR},
  volume    = {abs/2201.12150},
  year      = {2022},
  eprinttype = {arXiv}
}

@article{silver2016mastering,
  title={Mastering the game of {G}o with deep neural networks and tree search},
  author={Silver, David and Huang, Aja and Maddison, Chris J and Guez, Arthur and Sifre, Laurent and Van Den Driessche, George and Schrittwieser, Julian and Antonoglou, Ioannis and Panneershelvam, Veda and Lanctot, Marc and others},
  journal={Nature},
  volume={529},
  number={7587},
  pages={484--489},
  year={2016},
  publisher={Nature Publishing Group}
}

@article{vanschoren2014openml,
  title={OpenML: networked science in machine learning},
  author={Vanschoren, Joaquin and Van Rijn, Jan N and Bischl, Bernd and Torgo, Luis},
  journal={ACM SIGKDD Explorations Newsletter},
  volume={15},
  number={2},
  pages={49--60},
  year={2014},
  publisher={ACM New York, NY, USA}
}

@article{vinyals2016matching,
  title={Matching networks for one shot learning},
  author={Vinyals, Oriol and Blundell, Charles and Lillicrap, Timothy and Wierstra, Daan and others},
  journal={Advances in neural information processing systems},
  volume={29},
  pages={3630--3638},
  year={2016}
}

@book{witten2005practical,
  title={Practical machine learning tools and techniques},
  author={Witten, Ian H and Frank, Eibe and Hall, Mark A and Pal, Christopher J.},
  edition={4},
  year={2016},
  publisher={Elsevier Science \& Technology}
}

@InProceedings{Jin:2014,
author="Gu, Yingjie
and Jin, Zhong
and Chiu, Steve C.",
title="Combining Active Learning and Semi-supervised Learning Using Local and Global Consistency",
booktitle="Neural Information Processing",
year="2014",
publisher="Springer",
pages="215--222"
}

@article{Camargo:2020,
    author = {Camargo, Guilherme AND Bugatti, Pedro H. AND Saito, Priscila T. M.},
    journal = {PLOS ONE},
    publisher = {Public Library of Science},
    title = {Active semi-supervised learning for biological data classification},
    year = {2020},
    volume = {15},
    pages = {1-20},
    number = {8},
}

@inproceedings{khoreva_CVPR17,
 title={Simple Does It: Weakly Supervised Instance and Semantic Segmentation},
 author={A. Khoreva and R. Benenson and J. Hosang and M. Hein and B. Schiele},
 booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
 year={2017}
 }
 
 @inproceedings{Nowak:2010,
author = {Nowak, Stefanie and R\"{u}ger, Stefan},
title = {How Reliable Are Annotations via Crowdsourcing: A Study about Inter-Annotator Agreement for Multi-Label Image Annotation},
year = {2010},
booktitle = {Proceedings of the International Conference on Multimedia Information Retrieval},
pages = {557–566}
}

@INPROCEEDINGS{8462493,
  author={Maroto, Javier and Ortega, Antonio},
  booktitle={IEEE International Conference on Acoustics, Speech and Signal Processing}, 
  title={Efficient Worker Assignment in Crowdsourced Data Labeling Using Graph Signal Processing}, 
  year={2018},
  pages={2271-2275}
}

@article{gu2019understanding,
    title={Understanding Bias in Machine Learning},
    author={Jindong Gu and Daniela Oelke},
    year={2019},
    journal   = {CoRR},
    volume    = {abs/1909.01866},    
    primaryClass={cs.LG}
}

@inproceedings{Bird:2019:FML,
 author = {Bird, Sarah and Kenthapadi, Krishnaram and Kiciman, Emre and Mitchell, Margaret},
 title = {Fairness-Aware Machine Learning: Practical Challenges and Lessons Learned},
 booktitle = {International Conference on Web Search and Data Mining},
 year = {2019},
 pages = {834--835},
 numpages = {2}
}

@article{Dekel:2020,
author = {Dekel, Ron and Sagi, Dov},
year = {2020},
pages = {59},
title = {Perceptual bias is reduced with longer reaction times during visual discrimination},
volume = {3},
journal = {Communications Biology},
doi = {10.1038/s42003-020-0786-7}
}

@ARTICLE{Dimara:2020,
  author={E. {Dimara} and S. {Franconeri} and C. {Plaisant} and A. {Bezerianos} and P. {Dragicevic}},
  journal={IEEE Transactions on Visualization and Computer Graphics}, 
  title={A Task-Based Taxonomy of Cognitive Biases for Information Visualization}, 
  year={2020},
  volume={26},
  number={2},
  pages={1413-1432},
}

@article{todorov:2019:gender,
author = {DongWon Oh and Elinor A. Buck and Alexander Todorov},
title ={Revealing Hidden Gender Biases in Competence Impressions of Faces},
journal = {Psychological Science},
volume = {30},
number = {1},
pages = {65-79},
year = {2019}
}

@article{Talamas:2016,
    author = {Talamas, Sean N. AND Mavor, Kenneth I. AND Perrett, David I.},
    journal = {PLOS ONE},
    publisher = {Public Library of Science},
    title = {Blinded by Beauty: Attractiveness Bias and Accurate Perceptions of Academic Performance},
    year = {2016},
    month = {},
    volume = {11},
    number = {2},
    pages = {1-18}
}

@article{jacques:TAC:2019,
  author    = {Julio C. S. {Jacques Junior} and
               Yagmur G{\"{u}}{\c{c}}l{\"{u}}t{\"{u}}rk and
               Marc P{\'{e}}rez and
               Umut G{\"{u}}{\c{c}}l{\"{u}} and
               Carlos And{\'{u}}jar and
               Xavier Bar{\'{o}} and
               Hugo Jair Escalante and
               Isabelle Guyon and
               Marcel A. J. van Gerven and
               Rob van Lier and
               Sergio Escalera},
  title     = {First Impressions: {A} Survey on Vision-Based Apparent Personality
               Trait Analysis},
  journal   = {IEEE Transactions on Affective Computing (TAC)},
  year      = {2019}
}

@inproceedings{Shen:2019:ACII,
 author = {Judy Hanwen Shen and Agata Lapedriza and Rosalind W. Picard},
 title = {Unintentional affective priming during labeling may bias labels},
 pages={587-593},
 booktitle = {International Conference on Affective Computing and Intelligent Interaction},
 year = {2019}
 }
 
 @InProceedings{Hendricks_2018_ECCV,
author = {Anne Hendricks, Lisa and Burns, Kaylee and Saenko, Kate and Darrell, Trevor and Rohrbach, Anna},
title = {Women also Snowboard: Overcoming Bias in Captioning Models},
booktitle = {The European Conference on Computer Vision (ECCV)},
month = {September},
year = {2018}
}

@INPROCEEDINGS{Torralba:cvpr:2011,
author={A. {Torralba} and A. A. {Efros}},
booktitle={IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
title={Unbiased look at dataset bias},
year={2011},
pages={1521-1528}
}

@InProceedings{pmlr-v81-buolamwini18a,
  title = 	 {Gender Shades: Intersectional Accuracy Disparities in Commercial Gender Classification},
  author = 	 {Joy Buolamwini and Timnit Gebru},
  booktitle = 	 {Conference on Fairness, Accountability and Transparency},
  pages = 	 {77--91},
  year = 	 {2018},
  volume = 	 {81}
}

@article{Jiang:2019,
  author    = {Heinrich Jiang and
               Ofir Nachum},
  title     = {Identifying and Correcting Label Bias in Machine Learning},
  journal   = {CoRR},
  volume    = {abs/1901.04966},
  year      = {2019},
  archivePrefix = {arXiv},
  eprint    = {1901.04966}
}

@InProceedings{Yucer_2020_CVPR_Workshops,
author = {Yucer, Seyma and Akcay, Samet and Al-Moubayed, Noura and Breckon, Toby P.},
title = {Exploring Racial Bias Within Face Recognition via Per-Subject Adversarially-Enabled Data Augmentation},
booktitle = {Conference on Computer Vision and Pattern Recognition (CVPR) Workshops},
year = {2020}
} 

@INPROCEEDINGS{Sixta:eccvw:2020,
author="Tomáš Sixta and Julio C. S. Jacques Junior and Pau Buch-Cardona and Eduard Vazquez and Sergio Escalera",
bookTitle="European Conference on Computer Vision Workshop (ECCVW)",
title="FairFace Challenge at ECCV 2020: Analyzing Bias in Face Recognition",
year="2020",
}

@InProceedings{Quadrianto_2019_CVPR,
author = {Quadrianto, Novi and Sharmanska, Viktoriia and Thomas, Oliver},
title = {Discovering Fair Representations in the Data Domain},
booktitle = {IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
month = {},
pages = {8219-8228},
year = {2019}
} 

@InProceedings{Robinson_2020_CVPR_Workshops,
author = {Robinson, Joseph P. and Livitz, Gennady and Henon, Yann and Qin, Can and Fu, Yun and Timoner, Samson},
title = {Face Recognition: Too Bias, or Not Too Bias?},
booktitle = {Conference on Computer Vision and Pattern Recognition (CVPR) Workshops},
pages={1-10},
year = {2020}
}

@inproceedings{Yan:ICMI:2020,
author = {Yan, Shen and Huang, Di and Soleymani, Mohammad},
title = {Mitigating Biases in Multimodal Personality Assessment},
year = {2020},
//publisher = {Association for Computing Machinery},
//address = {New York, NY, USA},
//url = {https://doi.org/10.1145/3382507.3418889},
//doi = {10.1145/3382507.3418889},
booktitle = {International Conference on Multimodal Interaction (ICMI)},
pages = {361–369}
}

@INPROCEEDINGS{Escalante:IJCNN:2017,
author={H. J. {Escalante} and I. {Guyon} and S. {Escalera} and J. C. S. {Jacques Junior} and M. {Madadi} and X. {Baró} and S. {Ayache} and E. {Viegas} and Y. {Güçlütürk} and U. {Güçlü} and M. A. J. {van Gerven} and R. {van Lier}},
booktitle={International Joint Conference on Neural Networks (IJCNN)},
title={Design of an explainable machine learning challenge for video interviews},
year={2017},
pages={3688-3695}
}

@InProceedings{Park:CVPR:2018,
author = {Huk Park, Dong and Anne Hendricks, Lisa and Akata, Zeynep and Rohrbach, Anna and Schiele, Bernt and Darrell, Trevor and Rohrbach, Marcus},
title = {Multimodal Explanations: Justifying Decisions and Pointing to the Evidence},
booktitle = {IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
pages={8779-8788},
year = {2018}
}


@article{dehghani2021benchmark,
    title={The Benchmark Lottery}, 
    author={Mostafa Dehghani and Yi Tay and Alexey A. Gritsenko and Zhe Zhao and Neil Houlsby and Fernando Diaz and Donald Metzler and Oriol Vinyals},
    year={2021},
    journal   = {CoRR},
  volume    = {abs/2107.07002},
  archivePrefix = {arXiv},
  eprint    = {2107.07002}
}

@Article{electronics8080832,
AUTHOR = {Carvalho, Diogo V. and Pereira, Eduardo M. and Cardoso, Jaime S.},
TITLE = {Machine Learning Interpretability: A Survey on Methods and Metrics},
JOURNAL = {Electronics},
VOLUME = {8},
YEAR = {2019},
NUMBER = {8},
ARTICLE-NUMBER = {832},
ISSN = {2079-9292},
DOI = {10.3390/electronics8080832}
}

@inproceedings{DBLP:conf/cbms/CarmonaCC19,
  author    = {Fer Carmona and
               Jordi Conesa and
               Jordi Casas{-}Roma},
  title     = {Towards the Analysis of How Anonymization Affects Usefulness of Health
               Data in the Context of Machine Learning},
  booktitle = {International Symposium on Computer-Based Medical Systems},
  pages     = {604--608},
  year      = {2019},
  timestamp = {Sat, 05 Sep 2020 01:00:00 +0200},
  biburl    = {https://dblp.org/rec/conf/cbms/CarmonaCC19.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/mdai/Casas-RomaHT12,
  author    = {Jordi Casas{-}Roma and
               Jordi Herrera{-}Joancomart{\'{\i}} and
               Vicen{\c{c}} Torra},
  title     = {Comparing Random-Based and k-Anonymity-Based Algorithms for Graph
               Anonymization},
  booktitle = {Modeling Decisions for Artificial Intelligence},
  volume    = {7647},
  pages     = {197--209},
  publisher = {Springer},
  year      = {2012},
  timestamp = {Tue, 14 May 2019 10:00:52 +0200},
  biburl    = {https://dblp.org/rec/conf/mdai/Casas-RomaHT12.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{Sweeney2000,
	title = {Simple Demographics Often Identify People Uniquely},
	journal = {Carnegie Mellon University, Data Privacy},
	year = {2000},
	type = {Working paper},
	author = {Sweeney, Latanya}
}


@INPROCEEDINGS{Jacques:FG:2019,
  author={Jacques Junior, Julio C. S. and Ozcinar, Cagri and Marjanovic, Marina and Baró, Xavier and Anbarjafari, Gholamreza and Escalera, Sergio},
  booktitle={IEEE International Conference on Automatic Face Gesture Recognition (FG)}, 
  title={On the effect of age perception biases for real age regression}, 
  year={2019},
  pages={1-8},
  doi={10.1109/FG.2019.8756595}
}

@inproceedings{lopez2016chalearn,
  title={Cha{L}earn {LAP} 2016: First Round Challenge on First Impressions - Dataset and Results},
  author={Ponce-Lopez, VP and Chen, B and Places, A and Oliu, M and Corneanu, C and Baro, X and Escalante, HJ and Guyon, I and Escalera, S},
  booktitle={European Conference on Computer Vision Workshop (ECCVW)},
  year={2016},
  pages="400--418"
}

@article{liu2021winning,
  author={Liu, Zhengying and Pavao, Adrien and Xu, Zhen and Escalera, Sergio and Ferreira, Fabio and Guyon, Isabelle and Hong, Sirui and Hutter, Frank and Ji, Rongrong and Junior, Julio C. S. Jacques and Li, Ge and Lindauer, Marius and Luo, Zhipeng and Madadi, Meysam and Nierhoff, Thomas and Niu, Kangning and Pan, Chunguang and Stoll, Danny and Treguer, Sebastien and Wang, Jin and Wang, Peng and Wu, Chenglin and Xiong, Youcheng and Zela, Arbër and Zhang, Yang},
journal={IEEE Transactions on Pattern Analysis and Machine Intelligence}, 
title={Winning Solutions and Post-Challenge Analyses of the ChaLearn {AutoDL} Challenge 2019}, 
  year={2021},
  volume={43},
  number={9},
  pages={3108-3125}
}

@article{liu2019towards,
title = {Towards automated computer vision: analysis of the {AutoCV} challenges 2019},
journal = {Pattern Recognition Letters},
volume = {135},
pages = {196-203},
year = {2020},
issn = {0167-8655},
doi = {https://doi.org/10.1016/j.patrec.2020.04.030},
url = {https://www.sciencedirect.com/science/article/pii/S0167865520301525},
author = {Zhengying Liu and Zhen Xu and Sergio Escalera and Isabelle Guyon and Julio C.S. {Jacques Junior} and Meysam Madadi and Adrien Pavao and Sebastien Treguer and Wei-Wei Tu},
}

@article{DBLP:journals/corr/abs-1803-09010,
  author    = {Timnit Gebru and
               Jamie Morgenstern and
               Briana Vecchione and
               Jennifer Wortman Vaughan and
               Hanna M. Wallach and
               Hal Daum{\'{e}} III and
               Kate Crawford},
  title     = {Datasheets for Datasets},
  journal   = {CoRR},
  volume    = {abs/1803.09010},
  year      = {2018},
  url       = {http://arxiv.org/abs/1803.09010},
  eprinttype = {arXiv},
  eprint    = {1803.09010},
  timestamp = {Mon, 20 Aug 2018 15:16:09 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-1803-09010.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@Article{Shorten2019,
author={Shorten, Connor
and Khoshgoftaar, Taghi M.},
title={A survey on Image Data Augmentation for Deep Learning},
journal={Journal of Big Data},
year={2019},
volume={6},
number={1},
pages={60}
}

@article{Bender:2018,
    author = {Bender, Emily M. and Friedman, Batya},
    title = "{Data Statements for Natural Language Processing: Toward Mitigating System Bias and Enabling Better Science}",
    journal = {Transactions of the Association for Computational Linguistics},
    volume = {6},
    pages = {587-604},
    year = {2018},
    month = {12},
    eprint = {https://direct.mit.edu/tacl/article-pdf/doi/10.1162/tacl\_a\_00041/1567666/tacl\_a\_00041.pdf},
}

@article{10.1145/3448247,
author = {Gr\"{o}ger, Christoph},
title = {There is No AI without Data},
year = {2021},
issue_date = {November 2021},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
volume = {64},
number = {11},
issn = {0001-0782},
url = {https://doi.org/10.1145/3448247},
doi = {10.1145/3448247},
abstract = {Industry experiences on the data challenges of AI and the call for a data ecosystem for industrial enterprises.},
journal = {Commun. ACM},
month = {oct},
pages = {98–108},
numpages = {11}
}

@inproceedings{10.1145/3442188.3445918,
author = {Hutchinson, Ben and Smart, Andrew and Hanna, Alex and Denton, Emily and Greer, Christina and Kjartansson, Oddur and Barnes, Parker and Mitchell, Margaret},
title = {Towards Accountability for Machine Learning Datasets: Practices from Software Engineering and Infrastructure},
year = {2021},
booktitle = {ACM Conference on Fairness, Accountability, and Transparency (FAccT)},
pages = {560–575},
numpages = {16},
keywords = {datasets, requirements engineering, machine learning},
location = {Virtual Event, Canada}
}

@article{10.1145/3448247,
author = {Gr\"{o}ger, Christoph},
title = {There is No AI without Data},
year = {2021},
issue_date = {November 2021},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
volume = {64},
number = {11},
issn = {0001-0782},
url = {https://doi.org/10.1145/3448247},
doi = {10.1145/3448247},
abstract = {Industry experiences on the data challenges of AI and the call for a data ecosystem for industrial enterprises.},
journal = {Commun. ACM},
month = {oct},
pages = {98–108},
numpages = {11}
}

@phdthesis{liu:tel-03464519,
  TITLE = {{Automated Deep Learning : Principles and Practice}},
  AUTHOR = {Liu, Zhengying},
  URL = {https://tel.archives-ouvertes.fr/tel-03464519},
  NUMBER = {2021UPASG094},
  SCHOOL = {{Universit{\'e} Paris-Saclay}},
  YEAR = {2021},
  MONTH = Nov,
  KEYWORDS = {Automated machine learning ; Deep learning ; Experimental design ; Model selection ; Apprentissage automatique automatis{\'e} ; Apprentissage profond ; Plans d'experiences ; S{\'e}lection de mod{\`e}le},
  TYPE = {Theses},
  PDF = {https://tel.archives-ouvertes.fr/tel-03464519v2/file/95195_LIU_2021_archivage.pdf},
  HAL_ID = {tel-03464519},
  HAL_VERSION = {v2},
}

@book{10.5555/3152676,
author = {Voigt, Paul and Bussche, Axel von dem},
title = {The EU General Data Protection Regulation (GDPR): A Practical Guide},
year = {2017},
publisher = {Springer}
}

@inproceedings{Dosovitskiy17,
  title = { {CARLA}: {An} Open Urban Driving Simulator},
  author = {Alexey Dosovitskiy and German Ros and Felipe Codevilla and Antonio Lopez and Vladlen Koltun},
  booktitle = {Proceedings of the 1st Annual Conference on Robot Learning},
  pages = {1--16},
  year = {2017}
}

@INPROCEEDINGS{Abufadda:2021,
  author={Abufadda, Mohammad and Mansour, Khalid},
  booktitle={International Arab Conference on Information Technology (ACIT)}, 
  title={A Survey of Synthetic Data Generation for Machine Learning}, 
  year={2021},
  pages={1-7}
}

@book{Nikolenko:2021,
author = {Nikolenko, Sergey},
year = {2021},
title = {Synthetic Data for Deep Learning},
note      = {Part of the Springer Optimization and Its Applications book series (SOIA, volume 174)},
isbn = {978-3-030-75177-7},
publisher={Springer, Cham}
}

@InProceedings{Karras_2019_CVPR,
author = {Karras, Tero and Laine, Samuli and Aila, Timo},
title = {A Style-Based Generator Architecture for Generative Adversarial Networks},
booktitle = {Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR)},
month = {June},
year = {2019}
}

@INPROCEEDINGS{Queiroz:2010,
  author={Queiroz, Rossana and Cohen, Marcelo and Moreira, Juliano L. and Braun, Adriana and Jacques Junior, Julio C. and Musse, Soraia Raupp},
  booktitle={Conference on Graphics, Patterns and Images}, 
  title={Generating Facial Ground Truth with Synthetic Faces}, 
  year={2010},
  volume={},
  number={},
  pages={25-31}
}
  
@article{wood2021fake,
    title={Fake It Till You Make It: Face analysis in the wild using synthetic data alone},
    author={Erroll Wood and Tadas Baltru\v{s}aitis and Charlie Hewitt and Sebastian Dziadzio and Matthew Johnson and Virginia Estellers and Thomas J. Cashman and Jamie Shotton},
    year={2021},
    journal   = {CoRR},
    volume    = {abs/2109.15102},
    eprint={2109.15102},
    archivePrefix={arXiv},
    primaryClass={cs.CV}
}

@ARTICLE{Jacques:2010,
  author={Silveira Jacques Junior, Julio Cezar and Musse, Soraia Raupp and Jung, Claudio Rosito},
  journal={IEEE Signal Processing Magazine}, 
  title={Crowd Analysis Using Computer Vision Techniques}, 
  year={2010},
  volume={27},
  number={5},
  pages={66-77},
  doi={10.1109/MSP.2010.937394}
}

﻿@Article{Wang2021,
author={Wang, Qi
and Gao, Junyu
and Lin, Wei
and Yuan, Yuan},
title={Pixel-Wise Crowd Understanding via Synthetic Data},
journal={International Journal of Computer Vision},
year={2021},
month={Jan},
day={01},
volume={129},
number={1},
pages={225-245},
issn={1573-1405},
doi={10.1007/s11263-020-01365-4},
url={https://doi.org/10.1007/s11263-020-01365-4}
}

@article{musse:2007,
author = {Musse, Soraia R. and Jung, Cláudio R. and Jacques Jr, Julio C. S. and Braun, Adriana},
title = {Using computer vision to simulate the motion of virtual agents},
journal = {Computer Animation and Virtual Worlds},
volume = {18},
number = {2},
pages = {83-93},
keywords = {crowd simulation, panic situations, computer vision},
doi = {https://doi.org/10.1002/cav.163},
url = {https://onlinelibrary.wiley.com/doi/abs/10.1002/cav.163},
eprint = {https://onlinelibrary.wiley.com/doi/pdf/10.1002/cav.163},
year = {2007}
}

@INPROCEEDINGS{Khadka:2020,
  author={Khadka, A. and Remagnino, P. and Argyriou, V.},
  booktitle={IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP)}, 
  title={Synthetic Crowd and Pedestrian Generator for Deep Learning Problems}, 
  year={2020},
  pages={4052-4056},
  doi={10.1109/ICASSP40776.2020.9053301}
}

@article{YALE2020244,
title = {Generation and evaluation of privacy preserving synthetic health data},
journal = {Neurocomputing},
volume = {416},
pages = {244-255},
year = {2020},
issn = {0925-2312},
doi = {https://doi.org/10.1016/j.neucom.2019.12.136},
url = {https://www.sciencedirect.com/science/article/pii/S0925231220305117},
author = {Andrew Yale and Saloni Dash and Ritik Dutta and Isabelle Guyon and Adrien Pavao and Kristin P. Bennett},
keywords = {Synthetic data, Health data, Generative adversarial networks, Privacy},
}

@InProceedings{Kuppa:2021,
author="Kuppa, Aditya
and Aouad, Lamine
and Le-Khac, Nhien-An",
editor="Gruschka, Nils
and Antunes, Lu{\'i}s Filipe Coelho
and Rannenberg, Kai
and Drogkaris, Prokopios",
title="Towards Improving Privacy of Synthetic DataSets",
booktitle="Privacy Technologies and Policy",
year="2021",
publisher="Springer International Publishing",
address="Cham",
pages="106--119",
isbn="978-3-030-76663-4"
}

@article{Bellovin:2018,
author = {Bellovin, Steven and Dutta, Preetam and Reitinger, Nathan},
year = {2018},
month = {01},
pages = {},
title = {Privacy and Synthetic Datasets},
journal = {SSRN Electronic Journal},
doi = {10.2139/ssrn.3255766}
}

@article{breazeal2004social,
  title={Social interactions in {HRI}: the robot view},
  author={Breazeal, Cynthia},
  journal={IEEE Transactions on Systems, Man, and Cybernetics, Part C (Applications and Reviews)},
  volume={34},
  number={2},
  pages={181--186},
  year={2004},
  publisher={IEEE}
}

@article{LANGER2019231,
title = "Trust in socially assistive robots: Considerations for use in rehabilitation",
journal = "Neuroscience \& Biobehavioral Reviews",
volume = "104",
pages = "231 - 239",
year = "2019",
issn = "0149-7634",
//doi = "https://doi.org/10.1016/j.neubiorev.2019.07.014",
author = "Allison Langer and Ronit Feingold-Polak and Oliver Mueller and Philipp Kellmeyer and Shelly Levy-Tzedek",
}

@article{Matz:2017,
author = {S. C. Matz and M. Kosinski and G. Nave and D. J. Stillwell},
journal={Proceedings of the National Academy of Sciences of the United States of America (PNAS)},
year = {2017},
number = {48},
volume = {114},
pages = {12714-12719},
title = {Psychological targeting as an effective approach to digital mass persuasion},
}

@article{Mehrabi:2021,
author = {Mehrabi, Ninareh and Morstatter, Fred and Saxena, Nripsuta and Lerman, Kristina and Galstyan, Aram},
title = {A Survey on Bias and Fairness in Machine Learning},
year = {2021},
volume = {54},
number = {6},
journal = {ACM Computing Surveys},
pages={1-35}
}

@inproceedings{NIPS2017_a486cd07,
 author = {Kusner, Matt J and Loftus, Joshua and Russell, Chris and Silva, Ricardo},
 booktitle = {Advances in Neural Information Processing Systems (NeurIPS)},
 pages = {},
 title = {Counterfactual Fairness},
 volume = {30},
 year = {2017}
}

@article{ASHOKAN2021102646,
title = {Fairness metrics and bias mitigation strategies for rating predictions},
journal = {Information Processing and Management},
volume = {58},
number = {5},
pages = {102646},
year = {2021},
author = {Ashwathy Ashokan and Christian Haas}
}

@ARTICLE{Garcia-Molina:2018,
  author={Garcia-Molina, Hector and Joglekar, Manas and Marcus, Adam and Parameswaran, Aditya and Verroios, Vasilis},
  journal={IEEE Transactions on Knowledge and Data Engineering}, 
  title={Challenges in Data Crowdsourcing}, 
  year={2016},
  volume={28},
  number={4},
  pages={901-911}
}


@article{wilkinson_fair_2016,
	title = {The {FAIR} {Guiding} {Principles} for scientific data management and stewardship},
	volume = {3},
	language = {en},
	number = {1},
	urldate = {2022-05-05},
	journal = {Scientific Data},
	author = {Wilkinson, Mark D. and others},
	year = {2016},
	pages = {160018},
	file = {Wilkinson et al. - 2016 - The FAIR Guiding Principles for scientific data ma.pdf:/Users/romainegele/Zotero/storage/Z82WJR4K/Wilkinson et al. - 2016 - The FAIR Guiding Principles for scientific data ma.pdf:application/pdf},
}

@inproceedings{Miceli_FAccT21,
author = {Miceli, Milagros and Yang, Tianling and Naudts, Laurens and Schuessler, Martin and Serbanescu, Diana and Hanna, Alex},
title = {Documenting Computer Vision Datasets: An Invitation to Reflexive Data Practices},
year = {2021},
booktitle = {ACM Conference on Fairness, Accountability, and Transparency (FAccT)},
pages = {161–172},
numpages = {12},
keywords = {audits, accountability, datasheets for datasets, dataset documentation, transparency, training data, reflexivity, data annotation, machine learning},
location = {Virtual Event, Canada}
}

@article{Holland:2018,
  author    = {Sarah Holland and
               Ahmed Hosny and
               Sarah Newman and
               Joshua Joseph and
               Kasia Chmielinski},
  title     = {The Dataset Nutrition Label: {A} Framework To Drive Higher Data Quality
               Standards},
  journal   = {CoRR},
  volume    = {abs/1805.03677},
  year      = {2018},
  eprinttype = {arXiv},
  eprint    = {1805.03677},
  timestamp = {Mon, 13 Aug 2018 16:49:01 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-1805-03677.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@ARTICLE{Bhanot2021,
  title     = "The problem of fairness in synthetic healthcare data",
  author    = "Bhanot, Karan and Qi, Miao and Erickson, John S and Guyon,
               Isabelle and Bennett, Kristin P",
  journal   = "Entropy (Basel)",
  publisher = "MDPI AG",
  volume    =  23,
  number    =  9,
  pages     = "1165",
  month     =  sep,
  year      =  2021
}

@article{Bhanot:2022,
  author = {Bhanot, Karan and Baldini, Ioana and Wei, Dennis and Zeng, Jiaming and Bennett, Kristin P.},
  title = {Downstream Fairness Caveats with Synthetic Healthcare Data},
  journal   = {CoRR},
  volume    = {abs/2203.04462},
  publisher = {arXiv},
  year = {2022},
}

@InProceedings{Baiyu2016,
author="Chen, Baiyu
and Escalera, Sergio
and Guyon, Isabelle
and Ponce-L{\'o}pez, V{\'i}ctor
and Shah, Nihar
and Oliu Sim{\'o}n, Marc",
editor="Hua, Gang
and J{\'e}gou, Herv{\'e}",
title="Overcoming Calibration Problems in Pattern Labeling with Pairwise Ratings: Application to Personality Traits",
booktitle="Computer Vision -- ECCV 2016 Workshops",
year="2016",
publisher="Springer International Publishing",
address="Cham",
pages="419--432",
isbn="978-3-319-49409-8"
}

@inproceedings{Braylan2022,
author = {Braylan, Alexander and Alonso, Omar and Lease, Matthew},
title = {Measuring Annotator Agreement Generally across Complex Structured, Multi-Object, and Free-Text Annotation Tasks},
year = {2022},
booktitle = {Proceedings of the ACM Web Conference},
pages = {1720–1730},
numpages = {11},
keywords = {inter-annotator agreement, labeling, quality assurance, annotation},
location = {Virtual Event, Lyon, France}
}

@INPROCEEDINGS{Joo:ICCV:2015,
  author={Joo, Jungseock and Steen, Francis F. and Zhu, Song-Chun},
  booktitle={2015 IEEE International Conference on Computer Vision (ICCV)}, 
  title={Automated Facial Trait Judgment and Election Outcome Prediction: Social Dimensions of Face}, 
  year={2015},
  volume={},
  number={},
  pages={3712-3720},
  doi={10.1109/ICCV.2015.423}
}

@article{Checco2017, 
title={Let’s Agree to Disagree: Fixing Agreement Measures for Crowdsourcing}, 
volume={5}, 
number={1}, 
journal={Proceedings of the AAAI Conference on Human Computation and Crowdsourcing}, 
author={Checco, Alessandro and Roitero, Kevin and Maddalena, Eddy and Mizzaro, Stefano and Demartini, Gianluca}, 
year={2017}, 
pages={11-20} 
}

@Article{s22041596,
AUTHOR = {Rasmussen, Christoffer Bøgelund and Kirk, Kristian and Moeslund, Thomas B.},
TITLE = {The Challenge of Data Annotation in Deep Learning - A Case Study on Whole Plant Corn Silage},
JOURNAL = {Sensors},
VOLUME = {22},
YEAR = {2022},
NUMBER = {4},
ARTICLE-NUMBER = {1596},
PubMedID = {35214497}
}

@InProceedings{Liu_2018_CVPR,
author = {Liu, Bo and Wang, Xudong and Dixit, Mandar and Kwitt, Roland and Vasconcelos, Nuno},
title = {Feature Space Transfer for Data Augmentation},
booktitle = {IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
pages={9090-9098},
year = {2018}
} 

@article{Balestriero2022,
  title={The effects of regularization and data augmentation are class dependent},
  author={Balestriero, Randall and Bottou, Leon and LeCun, Yann},
  journal={Advances in Neural Information Processing Systems},
  volume={35},
  pages={37878--37891},
  year={2022}
}

@article{SEIJOPARDO201997,
title = {Biases in feature selection with missing data},
journal = {Neurocomputing},
volume = {342},
pages = {97-112},
year = {2019},
author = {Borja Seijo-Pardo and Amparo Alonso-Betanzos and Kristin P. Bennett and Verónica Bolón-Canedo and Julie Josse and Mehreen Saeed and Isabelle Guyon}
}

@inproceedings{SeijoPardo2018AnalysisOI,
  title={Analysis of imputation bias for feature selection with missing data},
  author={Borja Seijo-Pardo and Amparo Alonso-Betanzos and Kristin P. Bennett and Ver{\'o}nica Bol{\'o}n-Canedo and Isabelle Guyon and Julie Josse and Mehreen Saeed},
  booktitle={European Symposium on Artificial Neural Networks, Computational Intelligence and Machine Learning (ESANN)},
  year={2018},
pages = {655-660},
}

@INPROCEEDINGS{Guyon96whatsize,
    author = {Isabelle Guyon and John Makhoul and Richard Schwartz and Vladimir Vapnik},
    title = {What Size Test Set Gives Good Error Rate Estimates?},
    booktitle = {IEEE Transactions on Pattern Analysis and Machine Intelligence (TPAMI)},
    year = {1998},
    volume = {20},
    number = {01},
    pages = {52-64}
}

@INPROCEEDINGS{5767865,  author={Wang, Jiannan and Li, Guoliang and Fe, Jianhua},  booktitle={IEEE International Conference on Data Engineering},   title={Fast-join: An efficient method for fuzzy token matching based string similarity join},   year={2011},  volume={},  number={},  pages={458-469}
}


@InProceedings{pmlr-v130-lew21a,
  title = 	 { PClean: Bayesian Data Cleaning at Scale with Domain-Specific Probabilistic Programming },
  author =       {Lew, Alexander and Agrawal, Monica and Sontag, David and Mansinghka, Vikash},
  booktitle = 	 {International Conference on Artificial Intelligence and Statistics},
  series = 	 {Proceedings of Machine Learning Research (PMLR)},
  pages = 	 {1927--1935},
  year = 	 {2021},
  volume = 	 {130}
}

@article{wold1987principal,
  title={Principal component analysis},
  author={Wold, Svante and Esbensen, Kim and Geladi, Paul},
  journal={Chemometrics and intelligent laboratory systems},
  volume={2},
  number={1-3},
  pages={37--52},
  year={1987},
  publisher={Elsevier}
}

@article{guyon2003introduction,
  title={An introduction to variable and feature selection},
  author={Guyon, Isabelle and Elisseeff, Andr{\'e}},
  journal={Journal of machine learning research},
  volume={3},
  number={Mar},
  pages={1157--1182},
  year={2003}
}

@article{bourlard1988auto,
  title={Auto-association by multilayer perceptrons and singular value decomposition},
  author={Bourlard, Herv{\'e} and Kamp, Yves},
  journal={Biological cybernetics},
  volume={59},
  number={4},
  pages={291--294},
  year={1988},
  publisher={Springer}
}


@InProceedings{pmlr-v70-kusner17a,
  title = 	 {Grammar Variational Autoencoder},
  author =       {Matt J. Kusner and Brooks Paige and Jos{\'e} Miguel Hern{\'a}ndez-Lobato},
  booktitle = 	 {International Conference on Machine Learning},
  pages = 	 {1945--1954},
  year = 	 {2017},
  volume = 	 {70},
  series = 	 {Proceedings of Machine Learning Research (PMLR)}}

@article{mikolov2013efficient,
  title={Efficient estimation of word representations in vector space},
  author={Mikolov, Tomas and Chen, Kai and Corrado, Greg and Dean, Jeffrey},
  journal={arXiv preprint arXiv:1301.3781},
  year={2013}
}

@Inbook{tfidf,
editor="Sammut, Claude
and Webb, Geoffrey I.",
title="TF--IDF",
bookTitle="Encyclopedia of Machine Learning",
year="2010",
publisher="Springer",
address="Boston, MA",
pages="986--987",
isbn="978-0-387-30164-8"
}

@inproceedings{azizi2021big,
  title={Big self-supervised models advance medical image classification},
  author={Azizi, Shekoofeh and Mustafa, Basil and Ryan, Fiona and Beaver, Zachary and Freyberg, Jan and Deaton, Jonathan and Loh, Aaron and Karthikesalingam, Alan and Kornblith, Simon and Chen, Ting and others},
  booktitle={IEEE/CVF International Conference on Computer Vision (CVPR)},
  pages={3478--3488},
  year={2021}
}

@article{goel2020model,
  title={Model patching: Closing the subgroup performance gap with data augmentation},
  author={Goel, Karan and Gu, Albert and Li, Yixuan and R{\'e}, Christopher},
  journal={arXiv preprint arXiv:2008.06775},
  year={2020}
}

@inproceedings{pathak2016context,
  title={Context encoders: Feature learning by inpainting},
  author={Pathak, Deepak and Krahenbuhl, Philipp and Donahue, Jeff and Darrell, Trevor and Efros, Alexei A},
  booktitle={IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
  pages={2536--2544},
  year={2016}
}

@inproceedings{chen2020simple,
  title={A simple framework for contrastive learning of visual representations},
  author={Chen, Ting and Kornblith, Simon and Norouzi, Mohammad and Hinton, Geoffrey},
  booktitle={International conference on machine learning},
  pages={1597--1607},
  year={2020},
  series = {Proceedings of Machine Learning Research (PMLR)}
}

@article{bromley1993signature,
  title={Signature verification using a ``siamese'' time delay neural network},
  author={Bromley, Jane and Guyon, Isabelle and LeCun, Yann and S{\"a}ckinger, Eduard and Shah, Roopak},
  journal={Advances in Neural Information Processing Systems},
  volume={6},
pages={737–744},
  year={1993}
}

@article{weiss2016survey,
  title={A survey of transfer learning},
  author={Weiss, Karl and Khoshgoftaar, Taghi M and Wang, DingDing},
  journal={Journal of Big data},
  volume={3},
  number={1},
  pages={1--40},
  year={2016},
  publisher={SpringerOpen}
}

@ARTICLE{10.3389/fclim.2021.637037,
AUTHOR={Cooper, Caren B. and Rasmussen, Lisa M. and Jones, Elizabeth D.},   
TITLE={Perspective: The Power (Dynamics) of Open Data in Citizen Science},      
JOURNAL={Frontiers in Climate},      
VOLUME={3},           
YEAR={2021},      
DOI={10.3389/fclim.2021.637037},      
ISSN={2624-9553}
}

@book{10.7551/mitpress/11805.001.0001,
    author = {D'Ignazio, Catherine and Klein, Lauren F. },
    title = "{Data Feminism}",
    publisher = {The MIT Press},
    year = {2020},
    month = {03},
    isbn = {9780262358521},
    doi = {10.7551/mitpress/11805.001.0001},
    url = {https://doi.org/10.7551/mitpress/11805.001.0001},
}

@article{koch2021reduced,
  title={Reduced, reused and recycled: The life of a dataset in machine learning research},
  author={Koch, Bernard and Denton, Emily and Hanna, Alex and Foster, Jacob G},
  journal={arXiv preprint arXiv:2112.01716},
  year={2021}
}

@article{zhang2000flexible,
  title={A flexible new technique for camera calibration},
  author={Zhang, Zhengyou},
  journal={IEEE Transactions on Pattern Analysis and Machine Intelligence (TPAMI)},
  volume={22},
  number={11},
  pages={1330--1334},
  year={2000},
  publisher={IEEE}
}

@article{Benjamin2019TowardsSO,
  title={Towards Standardization of Data Licenses: The Montreal Data License},
  author={Misha Benjamin and Paul Gagnon and Negar Rostamzadeh and Christopher Joseph Pal and Yoshua Bengio and Alex Shee},
  journal={ArXiv},
  year={2019},
  volume={abs/1903.12262}
}

@techreport{krippendorff2011computing,
  title={Computing Krippendorff's alpha-reliability},
  author={Krippendorff, Klaus},
  year={2011},
  address = {Penn collection, Departmental Papers (ASC)}
}


@ARTICLE{7374704,
  author={Corneanu, Ciprian Adrian and Simón, Marc Oliu and Cohn, Jeffrey F. and Guerrero, Sergio Escalera},
  journal={IEEE Transactions on Pattern Analysis and Machine Intelligence}, 
  title={Survey on RGB, 3D, Thermal, and Multimodal Approaches for Facial Expression Recognition: History, Trends, and Affect-Related Applications}, 
  year={2016},
  volume={38},
  number={8},
  pages={1548-1568}
}

@article{kaufman2012leakage,
  title={Leakage in data mining: Formulation, detection, and avoidance},
  author={Kaufman, Shachar and Rosset, Saharon and Perlich, Claudia and Stitelman, Ori},
  journal={ACM Transactions on Knowledge Discovery from Data (TKDD)},
  volume={6},
  number={4},
  pages={1--21},
  year={2012},
  publisher={ACM New York, NY, USA}
}


@article {confounding_bias,
	author = {David Nunan and Jeffrey Aronson and Clare Bankhead},
	title = {Catalogue of bias: attrition bias},
	volume = {23},
	number = {1},
	pages = {21--22},
	year = {2018},
	publisher = {Royal Society of Medicine},
	eprint = {https://ebm.bmj.com/content/23/1/21.full.pdf},
	journal = {BMJ Evidence-Based Medicine}
}



@article{altmann2010permutation,
  title={Permutation importance: a corrected feature importance measure},
  author={Altmann, Andr{\'e} and Tolo{\c{s}}i, Laura and Sander, Oliver and Lengauer, Thomas},
  journal={Bioinformatics},
  volume={26},
  number={10},
  pages={1340--1347},
  year={2010},
  publisher={Oxford University Press}
}

@article{bhanot2021problem,
  title={The problem of fairness in synthetic healthcare data},
  author={Bhanot, Karan and Qi, Miao and Erickson, John S and Guyon, Isabelle and Bennett, Kristin P},
  journal={Entropy},
  volume={23},
  number={9},
  pages={1165},
  year={2021},
  publisher={MDPI}
}

@article{yale2020generation,
  title={Generation and evaluation of privacy preserving synthetic health data},
  author={Yale, Andrew and Dash, Saloni and Dutta, Ritik and Guyon, Isabelle and Pavao, Adrien and Bennett, Kristin P},
  journal={Neurocomputing},
  volume={416},
  pages={244--255},
  year={2020},
  publisher={Elsevier}
}

@article{pan2009survey,
  title={A survey on transfer learning},
  author={Pan, Sinno Jialin and Yang, Qiang},
  journal={IEEE Transactions on knowledge and data engineering},
  volume={22},
  number={10},
  pages={1345--1359},
  year={2009},
  publisher={IEEE}
}

@article{yeong2021sensor,
  title={Sensor and sensor fusion technology in autonomous vehicles: A review},
  author={Yeong, De Jong and Velasco-Hernandez, Gustavo and Barry, John and Walsh, Joseph},
  journal={Sensors},
  volume={21},
  number={6},
  pages={2140},
  year={2021},
  publisher={MDPI}
}

@article{bleiholder2009data,
  title={Data fusion},
  author={Bleiholder, Jens and Naumann, Felix},
  journal={ACM computing surveys (CSUR)},
  volume={41},
  number={1},
  pages={1--41},
  year={2009},
  publisher={ACM New York, NY, USA}
}


@article{carrion-2022,
title = {NeurIPS’22 Cross-Domain MetaDL competition:
Design and baseline results},
author = {Dustin Carri\'on and others},
year = {2022},
journal = {PMLR, to appear},
publisher = {ECML-PKDD 2022, Meta-Knowledge Transfer/Communication in Different Systems}
}

@book{montgomery2017design,
  title={Design and analysis of experiments},
  author={Montgomery, Douglas C},
  year={2017},
  publisher={John wiley \& sons}
}

@article{bergstra2012random,
  title   = {Random search for hyper-parameter optimization.},
  author  = {Bergstra, James and Bengio, Yoshua},
  journal = {Journal of machine learning research},
  volume  = {13},
  number  = {2},
  year    = {2012}
}

@article{settles2009active,
  title={Active learning literature survey},
  author={Settles, Burr},
  year={2009},
journal = {Computer Sciences Technical Report, 1648. University of Wisconsin-Madison, Department of Computer Sciences},
  publisher={University of Wisconsin-Madison Department of Computer Sciences}
}

@misc{google_robottxt_2022,
  title     = {Create a robots.txt file},
  url       = {https://developers.google.com/search/docs/advanced/robots/create-robots-txt},
  journal   = {Google},
  publisher = {Google},
  year      = {2022},
  month     = {Jul}
}

@book{emilio2013data,
author = {Emilio, Maurizio Di Paolo},
title = {Data Acquisition Systems: From Fundamentals to Applied Design},
year = {2013},
isbn = {1461442133},
publisher = {Springer},
}



@article{gray1998quantization,
  title={Quantization},
  author={Gray, Robert M. and Neuhoff, David L.},
  journal={IEEE Transactions on Information Theory},
  volume={44},
  number={6},
  pages={2325--2383},
  year={1998},
  publisher={IEEE}
}

@book{higgins1996sampling,
  title={Sampling theory in Fourier and signal analysis: foundations},
  author={Higgins, John Rowland},
  year={1996},
  isbn={0198596995},
  publisher={Oxford Science Publications}
}

@article{ieee754,
  journal={IEEE Std 754-2019 (Revision of IEEE 754-2008)}, 
  title={IEEE Standard for Floating-Point Arithmetic}, 
  year={2019},
  volume={},
  number={},
  doi={10.1109/IEEESTD.2019.8766229},

  pages={1-84},

}
  
@article{zhou2018brief,
  title     = {A brief introduction to weakly supervised learning},
  author    = {Zhou, Zhi-Hua},
  journal   = {National science review},
  volume    = {5},
  number    = {1},
  pages     = {44--53},
  year      = {2018},
  publisher = {Oxford University Press}
}

@inproceedings{ratner2017snorkel,
  title        = {Snorkel: Rapid training data creation with weak supervision},
  author       = {Ratner, Alexander and Bach, Stephen H and Ehrenberg, Henry and Fries, Jason and Wu, Sen and R{\'e}, Christopher},
  booktitle    = {Proceedings of the VLDB Endowment. International Conference on Very Large Data Bases},
  volume       = {11},
  number       = {3},
  pages        = {269–282},
  year         = {2017}
}

@article{ridzuan2019review,
  title={A review on data cleansing methods for big data},
  author={Ridzuan, Fakhitah and Zainon, Wan Mohd Nazmee Wan},
  journal={Procedia Computer Science},
  volume={161},
  pages={731--738},
  year={2019},
  publisher={Elsevier}
}

@book{van2018flexible,
  title={Flexible imputation of missing data},
  author={Van Buuren, Stef},
  year={2018},
  publisher={CRC press}
}


@inbook{guyon1996discovering,
author = {Guyon, Isabelle and Matic, Nada and Vapnik, Vladimir},
title = {Discovering informative patterns and data cleaning},
year = {1996},
publisher = {American Association for Artificial Intelligence},
address = {USA},
booktitle = {Advances in Knowledge Discovery and Data Mining},
pages = {181–203},
numpages = {23}
}

@article{survey_datafusion_ml,
title = {A survey on machine learning for data fusion},
journal = {Information Fusion},
volume = {57},
pages = {115-129},
year = {2020},
author = {Tong Meng and Xuyang Jing and Zheng Yan and Witold Pedrycz},
keywords = {Data fusion, Machine learning, Fusion methods, Fusion criteria},
abstract = {Data fusion is a prevalent way to deal with imperfect raw data for capturing reliable, valuable and accurate information. Comparing with a range of classical probabilistic data fusion techniques, machine learning method that automatically learns from past experiences without explicitly programming, remarkably renovates fusion techniques by offering the strong ability of computing and predicting. Nevertheless, the literature still lacks a thorough review of the recent advances of machine learning for data fusion. Therefore, it is beneficial to review and summarize the state of the art in order to gain a deep insight on how machine learning can benefit and optimize data fusion. In this paper, we provide a comprehensive survey on data fusion methods based on machine learning. We first offer a detailed introduction to the background of data fusion and machine learning in terms of definitions, applications, architectures, processes, and typical techniques. Then, we propose a number of requirements and employ them as criteria to review and evaluate the performance of existing fusion methods based on machine learning. Through the literature review, analysis and comparison, we finally come up with a number of open issues and propose future research directions in this field.}
}

@article{zheng2015methodologies,
  title={Methodologies for cross-domain data fusion: An overview},
  author={Zheng, Yu},
  journal={IEEE transactions on big data},
  volume={1},
  number={1},
  pages={16--34},
  year={2015},
  publisher={IEEE}
}

@inproceedings{killamsetty2021grad,
  title={Grad-match: Gradient matching based data subset selection for efficient deep model training},
  author={Killamsetty, Krishnateja and Durga, S and Ramakrishnan, Ganesh and De, Abir and Iyer, Rishabh},
  booktitle={International Conference on Machine Learning},
  pages={5464--5474},
  year={2021},
  series = 	 {Proceedings of Machine Learning Research (PMLR)}
}


@inproceedings{NIPS2013_559cb990,
 author = {Bengio, Yoshua and Yao, Li and Alain, Guillaume and Vincent, Pascal},
 booktitle = {Advances in Neural Information Processing Systems},
 pages = {},
 title = {Generalized Denoising Auto-Encoders as Generative Models},
 volume = {26},
 year = {2013}
}

@article{kingma2013auto,
  title   = {Auto-encoding variational bayes},
  author  = {Kingma, Diederik P and Welling, Max},
  journal = {arXiv preprint arXiv:1312.6114},
  year    = {2013}
}

@ARTICLE{4767965,  author={Arun, K. S. and Huang, T. S. and Blostein, S. D.},  journal={IEEE Transactions on Pattern Analysis and Machine Intelligence (TPAMI)},   title={Least-Squares Fitting of Two 3-D Point Sets},   year={1987},  volume={9},  number={5},  pages={698-700}
}

@book{10.1093/acprof:oso/9780198510581.001.0001,
    author = {Gower, John C and Dijksterhuis, Garmt B},
    title = "{Procrustes Problems}",
    publisher = {Oxford University Press},
    year = {2004},
    isbn = {9780198510581}
}


@article{hernandez1998real,
  title={Real-world data is dirty: Data cleansing and the merge/purge problem},
  author={Hern{\'a}ndez, Mauricio A and Stolfo, Salvatore J},
  journal={Data mining and knowledge discovery},
  volume={2},
  number={1},
  pages={9--37},
  year={1998},
  publisher={Springer}
}

@article{yen2009cluster,
  title={Cluster-based under-sampling approaches for imbalanced data distributions},
  author={Yen, Show-Jane and Lee, Yue-Shi},
  journal={Expert Systems with Applications},
  volume={36},
  number={3},
  pages={5718--5727},
  year={2009},
  publisher={Elsevier}
}

@article{garcia2012effectiveness,
  title={On the effectiveness of preprocessing methods when dealing with different levels of class imbalance},
  author={Garc{\'\i}a, Vicente and S{\'a}nchez, Jos{\'e} Salvador and Mollineda, Ram{\'o}n Alberto},
  journal={Knowledge-Based Systems},
  volume={25},
  number={1},
  pages={13--21},
  year={2012},
  publisher={Elsevier}
}

@article{pollard1982quantization,
  title={Quantization and the method of k-means},
  author={Pollard, David},
  journal={IEEE Transactions on Information theory},
  volume={28},
  number={2},
  pages={199--205},
  year={1982},
  publisher={IEEE}
}

@article{devlin2018bert,
  title   = {Bert: Pre-training of deep bidirectional transformers for language understanding},
  author  = {Devlin, Jacob and Chang, Ming-Wei and Lee, Kenton and Toutanova, Kristina},
  journal = {arXiv preprint arXiv:1810.04805},
  year    = {2018}
}

 @article{radford2018improving,
  title     = {Improving language understanding by generative pre-training},
  author    = {Radford, Alec and Narasimhan, Karthik and Salimans, Tim and Sutskever, Ilya and others},
  year      = {2018},
  publisher = {OpenAI}
}

@inproceedings{pennington2014glove,
  title={Glove: Global vectors for word representation},
  author={Pennington, Jeffrey and Socher, Richard and Manning, Christopher D},
  booktitle={Proceedings of the Conference on Empirical Methods in Natural Language Processing (EMNLP)},
  pages={1532--1543},
  year={2014}
}

@article{bojanowski2017enriching,
  title={Enriching Word Vectors with Subword Information},
  author={Bojanowski, Piotr and Grave, Edouard and Joulin, Armand and Mikolov, Tomas},
  journal={Transactions of the Association for Computational Linguistics},
  volume={5},
  year={2017},
  pages={135--146}
}

@article{liu2019roberta,
  title={Roberta: A robustly optimized bert pretraining approach},
  author={Liu, Yinhan and Ott, Myle and Goyal, Naman and Du, Jingfei and Joshi, Mandar and Chen, Danqi and Levy, Omer and Lewis, Mike and Zettlemoyer, Luke and Stoyanov, Veselin},
  journal={arXiv preprint arXiv:1907.11692},
  year={2019}
}

@article{conneau2019unsupervised,
  title={Unsupervised cross-lingual representation learning at scale},
  author={Conneau, Alexis and Khandelwal, Kartikay and Goyal, Naman and Chaudhary, Vishrav and Wenzek, Guillaume and Guzm{\'a}n, Francisco and Grave, Edouard and Ott, Myle and Zettlemoyer, Luke and Stoyanov, Veselin},
  journal={arXiv preprint arXiv:1911.02116},
  year={2019}
}

@article{egele_dcaihyper_2022,
  title={Data Centric AI: Hype or Hallelujah},
  author={Egele, Romain and Jiang, Shengli and Prasanna, Balaprakash and Guyon, Isabelle},
  journal={Preprint},
  year={2022}
}

@misc{imagenet,
  doi = {10.48550/ARXIV.1409.0575},
  
  url = {https://arxiv.org/abs/1409.0575},
  
  author = {Russakovsky, Olga and Deng, Jia and Su, Hao and Krause, Jonathan and Satheesh, Sanjeev and Ma, Sean and Huang, Zhiheng and Karpathy, Andrej and Khosla, Aditya and Bernstein, Michael and Berg, Alexander C. and Fei-Fei, Li},
  
  keywords = {Computer Vision and Pattern Recognition (cs.CV), FOS: Computer and information sciences, FOS: Computer and information sciences, I.4.8; I.5.2},
  
  title = {ImageNet Large Scale Visual Recognition Challenge},
  
  publisher = {arXiv},
  
  year = {2014},
  
  copyright = {arXiv.org perpetual, non-exclusive license}
}

@inproceedings{agustsson2017appareal,
  title={Apparent and real age estimation in still images with deep residual regressors on APPA-REAL database.},
  author={E. Agustsson and R. Timofte and S. Escalera and X. Baro and I. Guyon and R. Rothe},
  booktitle={IEEE International Conference on Automatic Face and Gesture Recognition (FG)},
  year={2017},
pages = {87-94}
}


@InProceedings{Palmero_2021_WACV,
    author    = {Palmero, Cristina and Selva, Javier and Smeureanu, Sorina and Junior, Julio C. S. Jacques and Clapes, Albert and Mosegui, Alexa and Zhang, Zejian and Gallardo, David and Guilera, Georgina and Leiva, David and Escalera, Sergio},
    title     = {Context-Aware Personality Inference in Dyadic Scenarios: Introducing the UDIVA Dataset},
    booktitle = {Proceedings of the IEEE/CVF Winter Conference on Applications of Computer Vision (WACV) Workshops},
    month     = {January},
    year      = {2021},
    pages     = {1-12}
}

@article{10.1109/TPAMI.2018.2798607,
author = {Baltrusaitis, Tadas and Ahuja, Chaitanya and Morency, Louis-Philippe},
title = {Multimodal Machine Learning: A Survey and Taxonomy},
year = {2019},
issue_date = {February 2019},
publisher = {IEEE Computer Society},
address = {USA},
volume = {41},
number = {2},
issn = {0162-8828},
url = {https://doi.org/10.1109/TPAMI.2018.2798607},
doi = {10.1109/TPAMI.2018.2798607},
journal = {IEEE Transactions on Pattern Analysis and Machine Intelligence (TPAMI)},
month = {feb},
pages = {423–443},
numpages = {21}
}

@Article{Thudumu2020,
author={Thudumu, Srikanth
and Branch, Philip
and Jin, Jiong
and Singh, Jugdutt (Jack)},
title={A comprehensive survey of anomaly detection techniques for high dimensional big data},
journal={Journal of Big Data},
year={2020},
month={Jul},
day={02},
volume={7},
number={1},
pages={42},
issn={2196-1115},
doi={10.1186/s40537-020-00320-x},
url={https://doi.org/10.1186/s40537-020-00320-x}
}

@article{guardian20222022,
 author = "The Guardian",
 title = "{AI} programs exhibit racial and gender biases, research reveals",
 journal = " [ONLINE] {Accessed}",
 volume = "11/02/2024, Publication year",
 url={https://www.theguardian.com/technology/2017/apr/13/ai-programs-exhibit-racist-and-sexist-biases-research-reveals},
year="2017"
}

@article{post20222020,
  author = "The Washington Post",
 title = "Microsoft won’t sell police its facial-recognition technology, following similar moves by {Amazon} and {IBM}",
 journal = " [ONLINE] {Accessed}",
 volume = "11/02/2024, Publication year",
 url={https://www.washingtonpost.com/technology/2020/06/11/microsoft-facial-recognition/},
year="2020"
}

@article{hodge2004survey,
  title={A survey of outlier detection methodologies},
  author={Hodge, Victoria and Austin, Jim},
  journal={Artificial intelligence review},
  volume={22},
  number={2},
  pages={85--126},
  year={2004},
  publisher={Springer}
}

@article{hutter2021learning,
  title={Learning curve theory},
  author={Hutter, Marcus},
  journal={arXiv preprint arXiv:2102.04074},
  year={2021}
}

@article{sorscher2022beyond,
  title={Beyond neural scaling laws: beating power law scaling via data pruning},
  author={Sorscher, Ben and Geirhos, Robert and Shekhar, Shashank and Ganguli, Surya and Morcos, Ari S},
  journal={arXiv preprint arXiv:2206.14486},
  year={2022}
}

@article{paul2021deep,
  title={Deep learning on a data diet: Finding important examples early in training},
  author={Paul, Mansheej and Ganguli, Surya and Dziugaite, Gintare Karolina},
  journal={Advances in Neural Information Processing Systems},
  volume={34},
  pages={20596--20607},
  year={2021}
}

@article{toneva2018empirical,
  title={An empirical study of example forgetting during deep neural network learning},
  author={Toneva, Mariya and Sordoni, Alessandro and Combes, Remi Tachet des and Trischler, Adam and Bengio, Yoshua and Gordon, Geoffrey J},
  journal={arXiv preprint arXiv:1812.05159},
  year={2018}
}

@article{feldman2020neural,
  title={What neural networks memorize and why: Discovering the long tail via influence estimation},
  author={Feldman, Vitaly and Zhang, Chiyuan},
  journal={Advances in Neural Information Processing Systems},
  volume={33},
  pages={2881--2891},
  year={2020}
}

@article{meding2021trivial,
  title={Trivial or impossible--dichotomous data difficulty masks model differences (on ImageNet and beyond)},
  author={Meding, Kristof and Buschoff, Luca M Schulze and Geirhos, Robert and Wichmann, Felix A},
  journal={arXiv preprint arXiv:2110.05922},
  year={2021}
}

@article{REVISE_imagenet,
title = "REVISE: A Tool for Measuring and Mitigating Bias in Visual Datasets",
author = "Angelina Wang and Alexander Liu and Ryan Zhang and Anat Kleiman and Leslie Kim and Dora Zhao and Iroha Shirai and Arvind Narayanan and Olga Russakovsky",
year = "2022",
volume = "130",
pages = "1790--1810",
journal = "International Journal of Computer Vision",
publisher = "Springer Netherlands",
number = "7"
}

@book{barocas-hardt-narayanan,
  title = {Fairness and Machine Learning: Limitations and Opportunities},
  author = {Solon Barocas and Moritz Hardt and Arvind Narayanan},
  publisher = {MIT Press},
  year = {2023}
}



@inproceedings{10.1145/3278721.3278779,
author = {Zhang, Brian Hu and Lemoine, Blake and Mitchell, Margaret},
title = {Mitigating Unwanted Biases with Adversarial Learning},
year = {2018},
isbn = {9781450360128},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/3278721.3278779},
doi = {10.1145/3278721.3278779},
booktitle = {Proceedings of the 2018 AAAI/ACM Conference on AI, Ethics, and Society},
pages = {335–340},
numpages = {6},
location = {New Orleans, LA, USA},
series = {AIES '18}
}

@InProceedings{10.1007/978-3-540-79228-4_1,
author="Dwork, Cynthia",
title="Differential Privacy: A Survey of Results",
booktitle="Theory and Applications of Models of Computation",
year="2008",
publisher="Springer Berlin Heidelberg",
pages="1--19",
}

@article{10.1145/3439334,
author = {Steadman, Liam and Griffiths, Nathan and Jarvis, Stephen and Bell, Mark and Helman, Shaun and Wallbank, Caroline},
title = {KD-STR: A Method for Spatio-Temporal Data Reduction and Modelling},
year = {2021},
issue_date = {August 2021},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
volume = {2},
number = {3},
journal = {ACM/IMS Transactions on Data Science},
articleno = {17},
numpages = {31}
}

@InProceedings{Carreira_2017_CVPR,
author = {Carreira, Joao and Zisserman, Andrew},
title = {Quo Vadis, Action Recognition? A New Model and the Kinetics Dataset},
booktitle = {IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
 pages={4724-4733},
year = {2017}
}

@InProceedings{Tran_2018_CVPR,
author = {Tran, Du and Wang, Heng and Torresani, Lorenzo and Ray, Jamie and LeCun, Yann and Paluri, Manohar},
title = {A Closer Look at Spatiotemporal Convolutions for Action Recognition},
booktitle = {IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
pages = {6450-6459},
year = {2018}
}

@InProceedings{pmlr-v173-palmero22b,
  title = 	 {ChaLearn {LAP} Challenges on Self-Reported Personality Recognition and Non-Verbal Behavior Forecasting During Social Dyadic Interactions: Dataset, Design, and Results},
  author =       {Palmero, Cristina and Barquero, German and Jacques Junior, Julio C. S. and Clap{\'e}s, Albert and N{\'u}{\~n}ez, Johnny and Curto, David and Smeureanu, Sorina and Selva, Javier and Zhang, Zejian and Saeteros, David and Gallardo-Pujol, David and Guilera, Georgina and Leiva, David and Han, Feng and Feng, Xiaoxue and He, Jennifer and Tu, Wei-Wei and Moeslund, Thomas B. and Guyon, Isabelle and Escalera, Sergio},
  booktitle = 	 {Understanding Social Behavior in Dyadic and Small Group Interactions},
  pages = 	 {4--52},
  year = 	 {2022},
  volume = 	 {173},
  series = 	 {Proceedings of Machine Learning Research (PMLR)}
}
 
 
 @article{10.1145/3551390,
author = {Wan, Mingyang and Zha, Daochen and Liu, Ninghao and Zou, Na},
title = {In-Processing Modeling Techniques for Machine Learning Fairness: A Survey},
year = {2022},
journal = {ACM Transactions on Knowledge Discovery from Data}
}

@article{graph2vec_NarayananCVCLJ17,
  author    = {Annamalai Narayanan and
               Mahinthan Chandramohan and
               Rajasekar Venkatesan and
               Lihui Chen and
               Yang Liu and
               Shantanu Jaiswal},
  title     = {Graph2vec: Learning Distributed Representations of Graphs},
  journal   = {CoRR},
  volume    = {abs/1707.05005},
  year      = {2017},
  eprinttype = {arXiv},
  eprint    = {1707.05005},
  timestamp = {Thu, 02 Sep 2021 12:22:44 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/NarayananCVCLJ17.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{xia2016comprehensive,
  title={A comprehensive study of the past, present, and future of data deduplication},
  author={Xia, Wen and Jiang, Hong and Feng, Dan and Douglis, Fred and Shilane, Philip and Hua, Yu and Fu, Min and Zhang, Yucheng and Zhou, Yukun},
  journal={Proceedings of the IEEE},
  volume={104},
  number={9},
  pages={1681--1710},
  year={2016},
  publisher={IEEE}
}

@article{aif360-oct-2018,
    title = "{AI Fairness} 360:  An Extensible Toolkit for Detecting, Understanding, and Mitigating Unwanted Algorithmic Bias",
    author = {Rachel K. E. Bellamy and Kuntal Dey and Michael Hind and
	Samuel C. Hoffman and Stephanie Houde and Kalapriya Kannan and
	Pranay Lohia and Jacquelyn Martino and Sameep Mehta and
	Aleksandra Mojsilovic and Seema Nagar and Karthikeyan Natesan Ramamurthy and
	John Richards and Diptikalyan Saha and Prasanna Sattigeri and
	Moninder Singh and Kush R. Varshney and Yunfeng Zhang},
    year = {2018},
  journal   = {CoRR},
  volume    = {abs/1810.01943},
}


@inproceedings{kingma2016improved,
  title={Improved variational inference with inverse autoregressive flow},
  author={Kingma, Durk P and Salimans, Tim and Jozefowicz, Rafal and Chen, Xi and Sutskever, Ilya and Welling, Max},
  booktitle={Advances in Neural Information Processing Systems 29},
pages = {4743–4751},
  year={2016}
}

@article{goodfellow2020generative,
  title={Generative adversarial networks},
  author={Goodfellow, Ian and Pouget-Abadie, Jean and Mirza, Mehdi and Xu, Bing and Warde-Farley, David and Ozair, Sherjil and Courville, Aaron and Bengio, Yoshua},
  journal={Communications of the ACM},
  volume={63},
  number={11},
  pages={139--144},
  year={2020},
  publisher={ACM New York, NY, USA}
}

@article{JMLR:v18:16-365,
author  = {Guillaume  Lema{{\^i}}tre and Fernando Nogueira and Christos K. Aridas},
title   = {Imbalanced-learn: A Python Toolbox to Tackle the Curse of Imbalanced Datasets in Machine Learning},
journal = {Journal of Machine Learning Research},
year    = {2017},
volume  = {18},
number  = {17},
pages   = {1-5}
}

@article{mehrabi2021survey,
  title={A survey on bias and fairness in machine learning},
  author={Mehrabi, Ninareh and Morstatter, Fred and Saxena, Nripsuta and Lerman, Kristina and Galstyan, Aram},
  journal={ACM Computing Surveys (CSUR)},
  volume={54},
  number={6},
  pages={1--35},
  year={2021},
  publisher={ACM New York, NY, USA}
}

@inproceedings{tian2018eliminating,
  title={Eliminating background-bias for robust person re-identification},
  author={Tian, Maoqing and Yi, Shuai and Li, Hongsheng and Li, Shihua and Zhang, Xuesen and Shi, Jianping and Yan, Junjie and Wang, Xiaogang},
  booktitle={IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
  pages={5794--5803},
  year={2018}
}

@InProceedings{radioactive_sablayrolles_2020,
  title = 	 {Radioactive data: tracing through training},
  author =       {Sablayrolles, Alexandre and Douze, Matthijs and Schmid, Cordelia and Jegou, Herve},
  booktitle = 	 {International Conference on Machine Learning},
  pages = 	 {8326--8335},
  year = 	 {2020},
  volume = 	 {119},
  series = 	 {Proceedings of Machine Learning Research (PMLR)},
}



@INPROCEEDINGS{simsiam_chen_2020,
  author={Chen, Xinlei and He, Kaiming},
  booktitle={IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR)}, 
  title={Exploring Simple Siamese Representation Learning}, 
  year={2021},
  pages={15745-15753},
}


@article{dccheck_seedat_20222,
  author = {Seedat, Nabeel and Imrie, Fergus and van der Schaar, Mihaela},
  title = {{DC}-Check: A Data-Centric AI checklist to guide the development of reliable machine learning systems},
  publisher = {arXiv},
  year = {2022},
  journal   = {CoRR},
  volume    = {2211.05764},
  year      = {2022},
  eprinttype = {arXiv},
  copyright = {Creative Commons Attribution 4.0 International}
}

@article{harrison1978hedonic,
  title={Hedonic housing prices and the demand for clean air},
  author={Harrison Jr, David and Rubinfeld, Daniel L},
  journal={Journal of environmental economics and management},
  volume={5},
  number={1},
  pages={81--102},
  year={1978},
  publisher={Elsevier}
}

@article{torralba200880,
  title={80 million tiny images: A large data set for nonparametric object and scene recognition},
  author={Torralba, Antonio and Fergus, Rob and Freeman, William T},
  journal={IEEE Transactions on Pattern Analysis and Machine Intelligence (TPAMI)},
  volume={30},
  number={11},
  pages={1958--1970},
  year={2008},
  publisher={IEEE}
}



@inproceedings{gpt3,
 author = {Brown, Tom and others},
 booktitle = {Advances in Neural Information Processing Systems (NeurIPS)},
 pages = {1877--1901},
 title = {Language Models are Few-Shot Learners},
 volume = {33},
 year = {2020}
}




@InProceedings{Ajith:2023,
author="Ajith, Ashly
and Gopakumar, G.",
title="Domain Adaptation: A Survey",
booktitle="Computer Vision and Machine Intelligence - Lecture Notes in Networks and Systems",
year="2023",
vol="586",
publisher="Springer, Singapore",
pages="591--602"
}

@article{ZHAO2024122807,
title = {A comparison review of transfer learning and self-supervised learning: Definitions, applications, advantages and limitations},
journal = {Expert Systems with Applications},
volume = {242},
pages = {122807},
year = {2024},
author = {Zehui Zhao and Laith Alzubaidi and Jinglan Zhang and Ye Duan and Yuantong Gu}
}
